Ultimate periodicity of b-recognisable sets : a quasilinear procedure

It is decidable if a set of numbers, whose representation in a base b is a regular language, is ultimately periodic. This was established by Honkala in 1986. We give here a structural description of minimal automata that accept an ultimately periodic set of numbers. We then show that it can verified in linear time if a given minimal automaton meets this description. This thus yields a O(n log(n)) procedure for deciding whether a general deterministic automaton accepts an ultimately periodic set of numbers.

==> VCSG-Preferences.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-Preferences
%%
%% DESCRIPTION:  Initial setting of VauCanSon-G's parameters
%%
%  VCSG-Preferences.tex is required to initialize VauCanSon-G:
%  VauCanSon-G does not perform any initialisation.
%  The values set in this file are mainly those used in EAT
%  
%  The file can also be used as a template to write 
%  a customized style of Vaucanson.
%  
%  VauCanSon-G is cut into 3 main files :
%  VCSG-environment.tex,  VCSG-states.tex,  and VCSG-edges.tex
%  VCSG-Preferences.tex has 3 parts corresponding to each of these 
%  files; inside a part the initialisation follows the appearance of  
%  the parameters in the file
%%  
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%    2.0 - 041112
%    2.2 - 050727 -- 050818
%    2.3 - 060627; 060717
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-environment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Scaling matters}%%%%%  
% Inner parameters
\renewcommand{\LargeScale}{0.85}    %float : argument of a \scalebox
\renewcommand{\LargeScaleI}{1.18}
\renewcommand{\MediumScale}{0.6}    %float
\renewcommand{\MediumScaleI}{1.67}
\renewcommand{\SmallScale}{0.5}     %float
\renewcommand{\SmallScaleI}{2}
\renewcommand{\TinyScale}{0.42}     %float
\renewcommand{\TinyScaleI}{2.38}
%
\MediumPictures
\FixVCGridScale{1}
%%%%%\section{Picture directory}%%%%%
% \SetVCDirectory{}  % for record : the definition of \VCDirectory is 
%                    % an initialisation 
%%%%%\section{Picture framing}%%%%%
% Inner parameters
\setlength{\VCFrameLineWidth}{0.6pt}
\renewcommand{\VCFrameLineColor}{black}
\setlength{\VCGridLineWidth}{0.6pt}
\renewcommand{\VCGridLineColor}{black}
%
\SetVCBkgdStyle{solid} % Also set StateBkgd, SmallStateBkgd,
                       % SttBorderColor,EdgeLineBorderColor
\SetVCBkgdColor{white} % and DblEdgeLineColor
%
\HideFrame\HideGrid\HideName
%%%%%\section{Picture drawing call}%%%%%
\FixVerticalPlacement{0.5} %float 
%%%%%\section{VauCanSon-G modes}%%%%%
\Automata 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-states}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{node mode}%%%%%%
% \SizedNodes % for record; not necessary after the call to \Automata 
%%%%%\section{state size}%%%%%%
\setlength{\SmallStateDiameter}{.6cm}
\setlength{\MediumStateDiameter}{1cm}
\setlength{\LargeStateDiameter}{1.2cm}
% \FixStateSizes{.6cm}{.9cm}{1.2cm}{.3cm} would have the same effect
%
% \MediumStates postponed after the definition of loop geometry 
% parameters
%%%%%\section{state shape}%%%%%
\CircleStates
\SetOvalStateRatio{\GoldMeanI}
\SetRectangleStateRatio{\GoldMeanI}
%
\SharpStateCorners 
\StateCornerRoundingAbsolute
\SetStateCornerRelRadius{0}
\SetStateCornerRadius{0.2cm}
%%%%%\section{Hiding -- showing}%%%%%
\ShowStates
%%%%%\section{state background parameters}%%%%%
% for record: setting done when setting the Bkgd of the picture 
% \SetStateBkgdStyle{\VCBkgdStyle}\SetStateBkgdColor{\VCBkgdColor}
% \SetSmallStateBkgdStyle{\VCBkgdStyle}
% \SetSmallStateBkgdColor{\VCBkgdColor}
%%%%%\section{construction line parameters}%%%%%%
\renewcommand{\SqrSttCtrClr}{blue}
\renewcommand{\LblBxLnClr}{red}
\renewcommand{\PhtSttLnClr}{green}
\CtrBxLblOff
\CtrSqrSttOff
\CtrPhtSttOff
\setlength{\PhtSttCtr}{0pt} %%% 
%%%%%\section{state line parameters}%%%%%%
% Inner parameters
\renewcommand{\SttDimen}{outer}
\renewcommand{\SttDblLineDimen}{middle}
\setlength{\SttBorderWidth}{0pt}
% \renewcommand{\SttBorderColor}{\StateBkgdColor} for record
\FixStateLineDouble{0.6}{0.4}  
%%%%%\section{state line parameters}%%%%%%
\SetStateLineWidth{1.8pt}
\SetStateLineStyle{solid}
\SetStateLineColor{black}
%
\StateLineSimple
%%%%%\section{state label parameters}%%%%%
\RigidStateLabel\FloatingStateLabel\StateLabelInside
\SetStateLabelColor{black}
% \SetStateLabelScale{1.667} (set by the scale picture commands)
\SetStateLabelSize{\normalsize}
\StateLabelModeMath
\SetStateLabelStyle{}
\SetAsideLabelDirct{72}
\SetAsideLabelDistn{6pt}
%%% Variable States
% extra space between the label and the state line (to be fixed)
\setlength{\ExtraSpaceForCrcState}{4mm}
\setlength{\ExtraSpaceForOvlState}{2mm}
\setlength{\ExtraSpaceForRctState}{2mm}
% mode initialisation
\HorizontalStateVarMode\SelfAdjustState
%%% Sizeless States
\setlength{\VerySmallStateDiameter}{.3cm}
%%% Dimmed states
% \renewcommand{\DimStateLineStyle}{solid} 
% \renewcommand{\DimStateLineCoef}{1} % 
% \renewcommand{\DimStateLineColor}{gray}
% \renewcommand{\DimStateLabelColor}{gray}
% \renewcommand{\DimStateBkgdColor}{white}
\SetDimStatePmts{solid}{1}{gray}{gray}{white}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-edges}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge label drawing macros
\renewcommand{\InOutLbl}[2]{#1\!\mid\! #2} % other ex: {(#1, #2)} 
\renewcommand{\IOL}[2]{#1\!\mid\! #2} % downward compatibility 
\renewcommand{\LblCnnct}{+}
%%% Edge drawing parameters
%%% Line
\SetEdgeLineWidth{1pt}			%% width (length param.)
\SetEdgeLineStyle{solid}		%% aspect
\SetEdgeLineColor{black}		%% color
\EdgeLineSimple
% double line the two coefficients have already been initialised in 
% VCSG-edges.tex in order to avoid deadlock; the call to 
% \FixEdgeLineDouble completes the initialisation
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
\SetDblEdgeLineColor{\VCBkgdColor} %% useless since it has 
              %% already been initialised with the picture background
% border
\EdgeLineBorderOff
\FixEdgeLineBorder{2}{\VCBkgdColor}		%% int,color : coef*\EdgeLineWidth -> width of border
%%% Edge arrow
\ArrowEdge				%% fix the style of arrows
% arrows on simple line 
\SetEdgeArrowWidthBase{2.5pt}
\SetEdgeArrowWidthCoef{2}
\SetEdgeArrowLengthCoef{1.4}
\SetEdgeArrowInsetCoef{0.1}
% idem  \SetEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
% arrows on double line 
\SetDblEdgeArrowWidthBase{2.5pt}
\SetDblEdgeArrowWidthCoef{1.6}
\SetDblEdgeArrowLengthCoef{1.3}
\SetDblEdgeArrowInsetCoef{0.1}
% idem  \SetDblEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
%%% Edge geometry parameters
\SetEdgeOffset{3pt}
\SetEdgeOffsetCoef{3}
\EdgeOffsetOff
\EdgeOffsetAbs
\SetForthBackEdgeOffsetCoef{2}% coef
\ForthBackOffsetOff
%
\NodeSeparationOff
\SetNodeSep{3pt}
%%% Edge label parameters
\EdgeLabelModeMath
\SetEdgeLabelSize{\normalsize}
\SetEdgeLabelStyle{}
\SetEdgeLabelColor{black}
\SetEdgeLabelScale{1.667}
%%% Edge label boxing parameters
\BoxedEdgeLabelOff
\renewcommand{\BxdEdgLblSep}{5}
\renewcommand{\BxdEdgLblBkg}{white}
\renewcommand{\BxdEdgLblWdt}{1}
\renewcommand{\BxdEdgLblStl}{solid}
\renewcommand{\BxdEdgLblCol}{black}
\renewcommand{\BxdEdgLblDbl}{false}
\renewcommand{\BxdEdgLblRnd}{0}
%%% Edge label geometry parameters
\DirectTransitions
\SetEdgLblPosit{.45}{.55}
\SetArcLblPosit{.4}{.6}
\SetLArcLblPosit{.4}{.6}
\SetLoopLblPosit{.25}{.75}
\SetCLoopLblPosit{.25}{.75}
%
\SetTransLabelSep{8pt}
%
\SwivelEdgeLabel
%%% Dimmed edges
% \renewcommand{\DimEdgeLineStyle}{solid} 
% \renewcommand{\DimEdgeLineCoef}{1.2} 
% \renewcommand{\DimEdgeLineColor}{gray}
% \renewcommand{\DimEdgeLabelColor}{gray}
\SetDimEdgePmts{solid}{1.2}{gray}{gray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\ArrowOnSmallState}{1.2} 		%float
\renewcommand{\ArrowOnMediumState}{1}		%float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnLargeState}{.8}		%float
% implicit parameter
\renewcommand{\InitialDir}{w}
\renewcommand{\FinalDir}{e}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arc geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetArcAngle{15}
\SetLArcAngle{30}
% Curvature
\SetArcCurvature{0.8}
\SetLArcCurvature{0.8}
% Offset
\SetArcOffset{1pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Loop geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetLoopAngle{30}
\SetCLoopAngle{22}
% Preset sizes
\renewcommand{\LoopOnSmallState}{9.6} 		%float
\renewcommand{\LoopOnMediumState}{7}		%float : curvature
\renewcommand{\LoopOnLargeState}{5.8} 		%float
\renewcommand{\CLoopOnSmallState}{12}		%float
\renewcommand{\CLoopOnMediumState}{8}		%float
\renewcommand{\CLoopOnLargeState}{6}		%float
% Offset
\SetLoopOffset{0pt}
%
\MediumStates
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\StateDimen}{outer}
\renewcommand{\StateDblDimen}{middle}
%
\renewcommand{\EdgeLabelPosit}{.45}   
\renewcommand{\EdgeLabelRevPosit}{.55}
\renewcommand{\ArcLabelPosit}{.40}
\renewcommand{\ArcLabelRevPosit}{.60}
\renewcommand{\LArcLabelPosit}{.40}
\renewcommand{\LArcLabelRevPosit}{.60}
\renewcommand{\LoopLabelPosit}{.25}
\renewcommand{\LoopLabelRevPosit}{.75}
\renewcommand{\CLoopLabelPosit}{.25}
\renewcommand{\CLoopLabelRevPosit}{.75}
%
\renewcommand{\LoopVarAngle}{28}
\renewcommand{\LoopOnVariableState}{5.1} 		%float
\renewcommand{\CLoopOnVariableState}{5.2}		%float
\setlength{\LoopVarOffset}{.7pt}
\renewcommand{\LoopOnVerySmallState}{15} 
% label position on initial-final arrow
\renewcommand{\InitStateLabelPosit}{.1}
\renewcommand{\InitStateLabelRevPosit}{.9}
\renewcommand{\FinalStateLabelPosit}{.9}
\renewcommand{\FinalStateLabelRevPosit}{.1}
%
\renewcommand{\ArrowOnVerySmallState}{5} 	%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \MediumStates
%%% Shape
%
%%% Variable States
\HorizontalStateVar\SelfAdjustState
%%% Showing -- hiding states
\ShowState
%%% Line
\renewcommand{\VSStateLineCoef}{.6} % coef. for very small state
%%% Background
%%% Label
%%% Label
\setlength{\VertexLineWidth}{0.6pt}             %% length
\renewcommand{\VertexLineColor}{black}        %% color
\renewcommand{\VertexBkgdStyle}{solid} 
\renewcommand{\VertexBkgdColor}{white}        %% color
\SetStateLabelColor{black}		
\renewcommand{\StateLabelScale}{1.7}
\renewcommand{\StateLabelSca}{1}% processing different from other parameters
\RigidLabel\FloatingLabel
%%% Initialisation
\RstState\RstVertex 
%%%%%%%%%%%%%%
%%%%%\section{edge parameters}%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetArcAngle{15}			%% int (degree)
\SetLArcAngle{30}			%% int (degree)
\SetArcCurvature{0.8}			%% float
\SetEdgeOffset{0pt}                     %% length
\SetArcOffset{1pt}			%% length
\SetLoopOffset{0pt}			%% length
\renewcommand{\ForthBackEdgeOffset}{5}	%% float : coef*\EdgeLineWidth -> offset
\FixEdgeBorder{2}{white}		%% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
%%%%%%%%%%%%%%
% ZZ aspect
%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}		% length : apparent diameter
\renewcommand{\ZZShape}{0.5}		% coef: opening of the ZZ
\SetZZLineWidth{1.7}			% float
\renewcommand{\TransLabelZZCoef}{0.6}	% float : coef*\ZZSize -> distance added for labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
% \SetEdgeArrowWidth{5pt}		%length of the edge arrow
% \SetEdgeArrowLengthCoef{1.4}		%float : coef*\EdgeArrowSizeDim width of EA
% \setlength{\EdgeDblArrowWidth}{5.5pt}		%length : size of EA for double transitions
% \renewcommand{\EdgeDblArrowLengthCoef}{1.7}	%int 
% \SetEdgeArrowInsetCoef{0.1}			%float : coef*\EdgeArrowSizeDim
% \SetEdgeArrowStyle{->}				%style (other styles : <-, |-|, -|,...)
% \renewcommand{\EdgeRevArrowStyle}{<-}           %style for reverse transitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState				%% PlainState
\MediumStates


==> VCSG-edges.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-edges.tex
%%
%% DESCRIPTION:     Commands for drawing edges
%%
%%   Auxiliary functions and variables called inside VauCanSon-G 
%%   PSTricks commands to be used inside pictures with VauCanSon-G's 
%%   syntax 
%%  
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%    2.3 - 060627    Copy of the "edge" part of VauCanSon-G 
%                    and adaptation to VCSG-states style
%    081228    transfer of macros from VCSG-functions 
%              transfer of PSTricks function Point to VCSG-functions  
%    091017    modif. EdgeOffset
%              modif. Edge composition label in order to take into 
%                     account \RigidEdgeLabel flag
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{Edge label drawing macros}%%%%%%%%
%%% Layout of compound labels (usage \InOutLbl{input}{output})
% to be initialised in preferences
\newcommand{\InOutLbl}[2]{}
\newcommand{\IOL}[2]{} % downward compatibility 
%%% Connector in lined or stacked labels 
\newcommand{\LblCnnct}{} % to be initialised in preferences
%%% Macros
%%% Stacked labels
\newcommand{\StackTwoLabels}[2]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{@{}c@{}}#1\\ #2 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabels}[3]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ #2 \\ #3 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
%%% Stacked labels with \LblCnnct
\newcommand{\StackTwoLabelsP}[2]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ \LblCnnct \\ #2 \end{array}%
   \renewcommand{\arraystretch}{1.333}}
\newcommand{\StackThreeLabelsP}[3]{%
   \renewcommand{\arraystretch}{0.75}%
   \begin{array}{c}#1\\ \LblCnnct\\#2\\ \LblCnnct\\#3\end{array}% 
   \renewcommand{\arraystretch}{1.333}}
%%% Lined up labels (with \LblCnnct)
\newcommand{\LineTwoLabelsP}[2]{#1 \LblCnnct #2} 
\newcommand{\LineThreeLabelsP}[3]{#1\LblCnnct #2\LblCnnct #3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\VarLoopOn}{\ChgLoopOffset{\LoopVarOff}%
   \ChgLoopSize{\LoopVarSi}%
   \ChgLoopAngle{\LoopVarAng}}
\newcommand{\VarLoopOff}{\RstLoopOffset \RstLoopSize \RstLoopAngle}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \section{Edge parameters}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsection{Edge drawing parameters}%%%%%%
%%% \subsubsection{Line}
\newlength{\EdgeLineWidth}\newlength{\EdgeLineWid}
\newcommand{\EdgeLineStyle}{}\newcommand{\EdgeLineSty}{}
\newcommand{\EdgeLineColor}{}\newcommand{\EdgeLineCol}{}
% changing/setting the width of edge line 
\newcommand{\ChgEdgeLineWidth}[1]% coefficient !
   {\setlength{\EdgeLineWid}{#1\EdgeLineWidth}%
    \SetEdgeLineBorderWidth%  %% update the width of border
    \SetDblEdgLineWD%    %% update the width of double line
    \SetEdgArrowWD%      %% see arrow section
    \SetDblEdgArrowWD%   %% see arrow section
    \SetEdgOffset%   %% see transition offset section
   }  
\newcommand{\RstEdgeLineWidth}{\ChgEdgeLineWidth{1}}
\newcommand{\SetEdgeLineWidth}[1]% ATTN the parameter is a length
   {\setlength{\EdgeLineWidth}{#1}\RstEdgeLineWidth}
% relative changing
\newcommand{\ChgRelEdgeLineWidth}[1]% coefficient !
   {\setlength{\EdgeLineWid}{#1\EdgeLineWid}%
    \SetEdgeLineBorderWidth%  %% update the width of border
    \SetDblEdgLineWD%    %% update the width of double line
    \SetEdgArrowWD%      %% see arrow section
    \SetDblEdgArrowWD%   %% see arrow section
    \SetEdgOffset%   %% see transition offset section
   }
% changing/setting the style of edge line 
\newcommand{\ChgEdgeLineStyle}[1]{\renewcommand{\EdgeLineSty}{#1}}  
\newcommand{\RstEdgeLineStyle}{\ChgEdgeLineStyle{\EdgeLineStyle}}
\newcommand{\SetEdgeLineStyle}[1]%
   {\renewcommand{\EdgeLineStyle}{#1}\RstEdgeLineStyle}
% changing/setting the color of edge line
\newcommand{\ChgEdgeLineColor}[1]{\renewcommand{\EdgeLineCol}{#1}}
\newcommand{\RstEdgeLineColor}{\ChgEdgeLineColor{\EdgeLineColor}}
\newcommand{\SetEdgeLineColor}[1]%
   {\renewcommand{\EdgeLineColor}{#1}\RstEdgeLineColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsubsection{Double line} (internal parameters)
% here we depart from the general policy of postponing initialization  
% setting macros for line width parameter call a macro that uses 
% double line coefficients and setting macro for double line 
% paramaters calls line width parameter.
% hence double line parameters are initialized here directly (ie without 
% using setting macros) and initialization is done normaly without 
% noticing the egg and chicken problem.
\newif\ifDblEdgLine
\newcommand{\DblEdgLine}{} 
\newcommand{\DblEdgLineCoef}{0.5} 
\newcommand{\DblEdgLineSep}{0.6} 
\newcommand{\DblEdgLineColor}{} %% Normaly set to picture bckg color
\newlength{\DblEdgLineWD} %% used to store the total width of double  
                          %% lines (see \SetDblEdgLineWD)
% internal function computes the total width of a double line
\newcommand{\SetDblEdgLineWD}% 
   {\setlength{\DblEdgLineWD}{\DblEdgLineCoef\EdgeLineWid}%
    \addtolength{\DblEdgLineWD}{\DblEdgLineCoef\EdgeLineWid}%
    \addtolength{\DblEdgLineWD}{\DblEdgLineSep\EdgeLineWid}}
% changing/setting the edge doubleline status
\newcommand{\EdgeLineDouble}%
   {\DblEdgLinetrue\renewcommand{\DblEdgLine}{true}}
\newcommand{\EdgeLineSimple}%
      {\DblEdgLinefalse\renewcommand{\DblEdgLine}{false}}
% changing/setting the edge doubleline parameters
\newcommand{\FixEdgeLineDouble}[2]%
   {\renewcommand{\DblEdgLineCoef}{#1}%
    \renewcommand{\DblEdgLineSep}{#2}
    \SetDblEdgLineWD\SetDblEdgArrowWD}
\newcommand{\SetDblEdgeLineColor}[1]%
   {\renewcommand{\DblEdgLineColor}{#1}}
\newcommand{\SetDblEdgeLineCoef}[1]%
   {\renewcommand{\DblEdgLineCoef}{#1}%
    \SetDblEdgLineWD\SetDblEdgArrowWD}
\newcommand{\SetDblEdgeLineSep}[1]%
   {\renewcommand{\DblEdgLineSep}{#1}%
    \SetDblEdgLineWD\SetDblEdgArrowWD}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsubsection{Border} (internal parameters)
% Border (of prescribed width and color) on both side of the line for 
% giving  the impression that one line passes above another. 
% May be useful when a transition crosses over another one.
\newif\ifEdgeLineBorder
\newlength{\EdgeLineBorderWidth}\newlength{\EdgeLineBorderWD}
\newcommand{\EdgeLineBorderCoef}{2} %% initialization for the same 
                                    %% reason as double line parameter
\newcommand{\EdgeLineBorderColor}{} %% normally same as picture bkgd 
                                    %% (\VCBkgdColor)
%%%%%
% \EdgeLineBorderWidth contains the width of the border if Border is 
% on. Must be updated  when \EdgeLineBorderCoef OR \EdgeLineWid are 
% changed.
% \EdgeLineBorderWD gives the border width to the style:
% 0pt when Border is off, \EdgeLineBorderWidth when Border is on.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  changing/setting macros 
% changing/setting the edge border status
\newcommand{\SetEdgeLineBorderWidth}% internal function  
   {\setlength{\EdgeLineBorderWidth}{\EdgeLineBorderCoef\EdgeLineWid}%
    \ifEdgeLineBorder%
       \setlength{\EdgeLineBorderWD}{\EdgeLineBorderWidth}%
    \fi}
\newcommand{\SetEdgeLineBorderCoef}[1]%
   {\renewcommand{\EdgeLineBorderCoef}{#1}\SetEdgeLineBorderWidth}
\newcommand{\SetEdgeLineBorderColor}[1]%
   {\renewcommand{\EdgeLineBorderColor}{#1}}
\newcommand{\FixEdgeLineBorder}[2]%
   {\SetEdgeLineBorderCoef{#1}%
    \SetEdgeLineBorderColor{#2}}
%
\newcommand{\EdgeLineBorderOn}%
   {\EdgeLineBordertrue%
    \setlength{\EdgeLineBorderWD}{\EdgeLineBorderWidth}}
\newcommand{\EdgeLineBorderOff}%
   {\EdgeLineBorderfalse
    \setlength{\EdgeLineBorderWD}{0pt}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsection{Edge arrow parameters}%%%%%%
% arrow style
\newcommand{\EdgeArrowStyle}{}\newcommand{\EdgeArrowSty}{}
\newcommand{\RevEdgArrowStyle}{}
% arrow dimensions
% as for double line parameters, we depart here from the general 
% policy of postponing initialization  
% setting macros for arrows use line width parameter and setting 
% macro for line width updates arrow dimension (width);
% hence arrow width parameters are initialized here directly (ie without
% using setting macros) and initialization is done normaly. 
\newlength{\EdgArrowWidthDim}
\newlength{\EdgArrowWDBase}       %% internal parameter;
\setlength{\EdgArrowWDBase}{2.5pt}  %% has to be set first
\newcommand{\EdgArrowWidthCoef}{2}
\newcommand{\EdgArrowLengthCoef}{}
\newcommand{\EdgArrowInsetCoef}{}
% arrow for double lines (we may want to have arrows on double lines of 
% (slightly) different shape)
\newlength{\DblEdgArrowWidthDim}
\newlength{\DblEdgArrowWDBase}       %% internal parameter;
\setlength{\DblEdgArrowWDBase}{2.5pt}  %% has to be set first
\newcommand{\DblEdgArrowWidthCoef}{1.6}
\newcommand{\DblEdgArrowLengthCoef}{}
\newcommand{\DblEdgArrowInsetCoef}{}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  setting macros 
% computing the arrow width (internal function)
% (must be called at every change of EdgeLineWidth)
% makes it necessary to initialize 
% Arrow coefficients BEFORE line width
\newcommand{\SetEdgArrowWD}% internal function
   {\setlength{\EdgArrowWidthDim}{\EdgArrowWDBase}%
    \addtolength{\EdgArrowWidthDim}{\EdgArrowWidthCoef\EdgeLineWid}}
\newcommand{\SetDblEdgArrowWD}% internal function
   {\setlength{\DblEdgArrowWidthDim}{\DblEdgArrowWDBase}%
    \addtolength{\DblEdgArrowWidthDim}%
                {\DblEdgArrowWidthCoef\DblEdgLineWD}}
% changing/setting arrow style 
\newcommand{\ChgEdgeArrowStyle}[1]{\renewcommand{\EdgeArrowSty}{#1}}
\newcommand{\RstEdgeArrowStyle}{\ChgEdgeArrowStyle{\EdgeArrowStyle}}
\newcommand{\SetEdgArwStyle}[1]%
   {\renewcommand{\EdgeArrowStyle}{#1}\RstEdgeArrowStyle}
%
\newcommand{\PlainEdge}%
   {\SetEdgArwStyle{-}%
    \renewcommand{\RevEdgArrowStyle}{-}}
\newcommand{\ArrowEdge}%
   {\SetEdgArwStyle{->}%
    \renewcommand{\RevEdgArrowStyle}{<-}}
\newcommand{\DblArrowEdge}%
   {\SetEdgArwStyle{->>}%
    \renewcommand{\RevEdgArrowStyle}{<<-}}
% changing/setting arrow dimensions
\newcommand{\SetEdgeArrowWidthBase}[1]% length!!
   {\setlength{\EdgArrowWDBase}{#1}%
    \SetEdgArrowWD}
\newcommand{\SetEdgeArrowWidthCoef}[1]%
   {\renewcommand{\EdgArrowWidthCoef}{#1}%
    \SetEdgArrowWD}
\newcommand{\SetEdgeArrowLengthCoef}[1]%
   {\renewcommand{\EdgArrowLengthCoef}{#1}}
\newcommand{\SetEdgeArrowInsetCoef}[1]%
   {\renewcommand{\EdgArrowInsetCoef}{#1}}
\newcommand{\FixEdgeArrowDimensions}[4]%
      {\SetEdgeArrowWidthBase{#1}%
       \SetEdgeArrowWidthCoef{#2}%
       \SetEdgeArrowLengthCoef{#3}%
       \SetEdgeArrowInsetCoef{#4}}
%
\newcommand{\SetDblEdgeArrowWidthBase}[1]% length!!
   {\setlength{\DblEdgArrowWDBase}{#1}%
    \SetDblEdgArrowWD}
\newcommand{\SetDblEdgeArrowWidthCoef}[1]%
   {\renewcommand{\DblEdgArrowWidthCoef}{#1}%
    \SetDblEdgArrowWD}
\newcommand{\SetDblEdgeArrowLengthCoef}[1]%
   {\renewcommand{\DblEdgArrowLengthCoef}{#1}}
\newcommand{\SetDblEdgeArrowInsetCoef}[1]%
   {\renewcommand{\DblEdgArrowInsetCoef}{#1}}
\newcommand{\SetDblEdgeArrowDimensions}[4]%
      {\SetDblEdgeArrowWidthBase{#1}%
       \SetDblEdgeArrowWidthCoef{#2}%
       \SetDblEdgeArrowLengthCoef{#3}%
       \SetDblEdgeArrowInsetCoef{#4}}
%
\newcommand{\ReverseTransitions}%
   {\ChgEdgeArrowStyle{\RevEdgArrowStyle}%
    \renewcommand{\EdgLblPos}{\EdgLblRevPosit}%
    \renewcommand{\ArcLblPos}{\ArcLblRevPosit}%
    \renewcommand{\LArcLblPos}{\LArcLblRevPosit}%
    \renewcommand{\LoopLblPos}{\LoopLblRevPosit}%
    \renewcommand{\CLoopLblPos}{\CLoopLblRevPosit}%
%     \renewcommand{\InitStateLblPos}{\InitStateLblRevPosit}%
%     \renewcommand{\FinalStateLblPos}{\FinalStateLblRevPosit}%
   }
\newcommand{\DirectTransitions}%
   {\RstEdgeArrowStyle%
    \renewcommand{\EdgLblPos}{\EdgLblPosit}%
    \renewcommand{\ArcLblPos}{\ArcLblPosit}%
    \renewcommand{\LArcLblPos}{\LArcLblPosit}%
    \renewcommand{\LoopLblPos}{\LoopLblPosit}%
    \renewcommand{\CLoopLblPos}{\CLoopLblPosit}%
%     \renewcommand{\InitStateLblPos}{\InitStateLblPosit}%
%     \renewcommand{\FinalStateLblPos}{\FinalStateLblPosit}%
   }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \section{Edge geometry parameters}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsubsection{Transition offset} 
% Implemented with a two-step process: on/off and a length. 
% This length is given as a multiple of EdgeLineWidth OR absolutely. 
% Moreover, for convenience AND upward compatilility, can be 
% superseeded by a ForthBackOffset command
\newif\ifEdgeOffset
\newif\ifEdgOffsetRel
\newlength{\EdgeOffset}\newlength{\EdgeOff}%
\newlength{\EdgOff}% buffer between \EdgeOffset and \EdgeOff
\newcommand{\EdgeOffsetCoef}{}% coef
\newcommand{\EdgOffCoef}{}% coef internal
\newcommand{\ForthBackEdgeOffsetCoef}{}% coef
% changing/setting transition offset
\newcommand{\ChgEdgeOffset}[1]%
   {\renewcommand{\EdgOffCoef}{#1}%
    \setlength{\EdgOff}{\EdgOffCoef\EdgeOffset}%
    \ifEdgeOffset\setlength{\EdgeOff}{\EdgOff}\fi%
    }
\newcommand{\RstEdgeOffset}{\ChgEdgeOffset{1}}
\newcommand{\SetEdgeOffset}[1]%
   {\EdgeOffsetAbs%
    \setlength{\EdgeOffset}{#1}\RstEdgeOffset}
\newcommand{\SetEdgeOffsetCoef}[1]%
   {\EdgeOffsetRel%
    \renewcommand{\EdgeOffsetCoef}{#1}%
    \setlength{\EdgeOffset}{\EdgeOffsetCoef\EdgeLineWid}\RstEdgeOffset}
%
\newcommand{\SetEdgOffset}% internal function, called when \EdgeLineWid changes
   {\ifEdgOffsetRel%
    \setlength{\EdgeOffset}{\EdgeOffsetCoef\EdgeLineWid}%
    \setlength{\EdgOff}{\EdgOffCoef\EdgeOffset}%
    \fi%
    \ifEdgeOffset
       \setlength{\EdgeOff}{\EdgOff}%
    \else
       \ifthenelse{\lengthtest{\EdgeOff > 0pt}}%if true \ForthBackOffset
          {\ForthBackOffsetOn}{}%              %is on
    \fi}
%
\newcommand{\EdgeOffsetOn}{\EdgeOffsettrue\setlength{\EdgeOff}{\EdgOff}}
\newcommand{\EdgeOffsetOff}{\EdgeOffsetfalse\setlength{\EdgeOff}{0pt}}
\newcommand{\EdgeOffsetRel}{\EdgOffsetReltrue}
\newcommand{\EdgeOffsetAbs}{\EdgOffsetRelfalse}
%
\newcommand{\SetForthBackEdgeOffsetCoef}[1]% 
   {\renewcommand{\ForthBackEdgeOffsetCoef}{#1}\ForthBackOffsetOn}%
\newcommand{\ForthBackOffsetOn}%
   {\EdgeOffsetOn\EdgeOffsetRel%   
    \SetEdgeOffsetCoef{\ForthBackEdgeOffsetCoef}}
\newcommand{\ForthBackOffsetOff}%
   {\ifEdgeOffset\setlength{\EdgeOff}{\EdgOff}%
    \else\setlength{\EdgeOff}{0pt}%
    \fi
    \EdgeOffsetOff}
%%%% Initialisation ??? 091017
\EdgeOffsetOff
\EdgeOffsetAbs
%%% \subsubsection{Node separation} 
% Distance between the node and the ends of transitions. 
% (not to be mistaken with the (state line) border). 
% Implemented with a two-step process: on/off and a length. 
% This length is given absolutely; would require more care and 
% procedures if it were a fonction of EdgeLineWidth for instance
\newlength{\NodeSep}\newlength{\NodeSP}%
\newlength{\NdSP}% buffer between \NodeSep and \NodeSP
% changing/setting node separation (normal procedure for length)
\newcommand{\ChgNodeSep}[1]%
   {\setlength{\NdSP}{#1\NodeSep}%
    \ifthenelse{\lengthtest{\NodeSP = 0pt}}% plays the role of a flag
       {}{\NodeSeparationOn}} 
\newcommand{\RstNodeSep}{\ChgNodeSep{1}} 
\newcommand{\SetNodeSep}[1]%
   {\setlength{\NodeSep}{#1}\RstNodeSep}
%
\newcommand{\NodeSeparationOn}{\setlength{\NodeSP}{\NdSP}}
\newcommand{\NodeSeparationOff}{\setlength{\NodeSP}{0pt}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \section{Edge label parameters}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% \subsection{\LaTeX parameters}
%%% label mode
\newcommand{\EdgLblMode}{} % Internal variable
% setting the label text mode %%% processed differently
\newcommand{\EdgeLabelModeMath}{\renewcommand{\EdgLblMode}{$}}%
\newcommand{\EdgeLabelModeText}{\renewcommand{\EdgLblMode}{}}%
%%% label size
\newcommand{\EdgeLabelSize}{}\newcommand{\EdgeLabelSz}{}
% changing/setting the label size
\newcommand{\ChgEdgeLabelSize}[1]{\renewcommand{\EdgeLabelSz}{#1}}
\newcommand{\RstEdgeLabelSize}{\ChgEdgeLabelSize{\EdgeLabelSize}}
\newcommand{\SetEdgeLabelSize}[1]%
    {\renewcommand{\EdgeLabelSize}{#1}\RstEdgeLabelSize}
%%% label style
\newcommand{\EdgeLabelStyle}{}\newcommand{\EdgeLabelSty}{}
% changing/setting the label style
\newcommand{\ChgEdgeLabelStyle}[1]{\renewcommand{\EdgeLabelSty}{#1}}
\newcommand{\RstEdgeLabelStyle}{\ChgEdgeLabelStyle{\EdgeLabelStyle}}
\newcommand{\SetEdgeLabelStyle}[1]%
    {\renewcommand{\EdgeLabelStyle}{#1}\RstEdgeLabelStyle}
%%% \subsection{graphical parameters}
%%% label colour
\newcommand{\EdgeLabelColor}{}\newcommand{\EdgeLabelCol}{}
% changing/setting the label color
\newcommand{\ChgEdgeLabelColor}[1]{\renewcommand{\EdgeLabelCol}{#1}}
\newcommand{\RstEdgeLabelColor}{\ChgEdgeLabelColor{\EdgeLabelColor}}
\newcommand{\SetEdgeLabelColor}[1]%
    {\renewcommand{\EdgeLabelColor}{#1}\RstEdgeLabelColor}
%%% label scale
\newcommand{\EdgeLabelScale}{}\newcommand{\EdgeLabelSca}{}
% changing/setting the label scale
\newcommand{\ChgEdgeLabelScale}[1]{\renewcommand{\EdgeLabelSca}{#1}}
\newcommand{\RstEdgeLabelScale}{\ChgEdgeLabelScale{1}}
\newcommand{\SetEdgeLabelScale}[1]%
   {\renewcommand{\EdgeLabelScale}{#1}\RstEdgeLabelScale}
%%% \subsection{Boxed label parameters}
\newif\ifVCBoxedEdgeLabel
\newcommand{\BoxedEdgeLabel}{}\newcommand{\BoxedEdgeLbl}{}
\newcommand{\BoxedEdgeLabelOn}{\VCBoxedEdgeLabeltrue}
\newcommand{\BoxedEdgeLabelOff}{\VCBoxedEdgeLabelfalse}
%
\newcommand{\BxdEdgLblSep}{}
\newcommand{\BxdEdgLblBkg}{}
\newcommand{\BxdEdgLblWdt}{}
\newcommand{\BxdEdgLblStl}{}
\newcommand{\BxdEdgLblCol}{}
\newcommand{\BxdEdgLblDbl}{}
\newcommand{\BxdEdgLblRnd}{}
%%% \subsection{geometric parameters}
%%% position on transitions
\newcommand{\EdgLblPosit}{}\newcommand{\EdgLblRevPosit}{}
\newcommand{\ArcLblPosit}{}\newcommand{\ArcLblRevPosit}{}
\newcommand{\LArcLblPosit}{}\newcommand{\LArcLblRevPosit}{}
\newcommand{\LoopLblPosit}{}\newcommand{\LoopLblRevPosit}{}
\newcommand{\CLoopLblPosit}{}\newcommand{\CLoopLblRevPosit}{}
\newcommand{\EdgLblPos}{}
\newcommand{\ArcLblPos}{}
\newcommand{\LArcLblPos}{}
\newcommand{\LoopLblPos}{}
\newcommand{\CLoopLblPos}{}
% changing/setting position on transitions ???
% \newcommand{\ChgEdgLblPosit}[1]{\renewcommand{\EdgLblPos}{#1}}  
% \newcommand{\RstEdgLblPosit}{\ChgEdgLblPosit{\EdgLblPosit}}
\newcommand{\SetEdgLblPosit}[2]%
   {\renewcommand{\EdgLblPosit}{#1}\renewcommand{\EdgLblPos}{#1}%
    \renewcommand{\EdgLblRevPosit}{#2}}
\newcommand{\SetArcLblPosit}[2]%
   {\renewcommand{\ArcLblPosit}{#1}\renewcommand{\ArcLblPos}{#1}%
    \renewcommand{\ArcLblRevPosit}{#2}}
\newcommand{\SetLArcLblPosit}[2]%
   {\renewcommand{\LArcLblPosit}{#1}\renewcommand{\LArcLblPos}{#1}%
    \renewcommand{\LArcLblRevPosit}{#2}}
\newcommand{\SetLoopLblPosit}[2]%
   {\renewcommand{\LoopLblPosit}{#1}\renewcommand{\LoopLblPos}{#1}%
    \renewcommand{\LoopLblRevPosit}{#2}}
\newcommand{\SetCLoopLblPosit}[2]%
   {\renewcommand{\CLoopLblPosit}{#1}\renewcommand{\CLoopLblPos}{#1}%
    \renewcommand{\CLoopLblRevPosit}{#2}}
%%% distance from transition
\newlength{\TransLabelSep}\newlength{\TransLabelSP}
% changing/setting distance from transition
\newcommand{\ChgTransLabelSep}[1]% coefficient !
   {\setlength{\TransLabelSP}{#1\TransLabelSep}}
\newcommand{\RstTransLabelSep}{\ChgTransLabelSep{1}}
\newcommand{\SetTransLabelSep}[1]% length !
   {\setlength{\TransLabelSep}{#1}\RstTransLabelSep}
\newcommand{\ChgRelTransLabelSep}[1]% coefficient !
      {\setlength{\TransLabelSP}{#1\TransLabelSP}}
%%% orientation
\newif\ifVCRigidEdgeLabel
\newcommand{\RigidEdgeLabel}{\VCRigidEdgeLabeltrue}
\newcommand{\SwivelEdgeLabel}{\VCRigidEdgeLabelfalse}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{dimmed edges}%%%%
%%%  Dimmed edges (e.g. for transitions to non accessible states)
\newcommand{\DimEdgeLineStyle}{} 
\newcommand{\DimEdgeLineCoef}{} 
\newcommand{\DimEdgeLineColor}{}
\newcommand{\DimEdgeLabelColor}{}
%%% establishing the dimmed style
\newcommand{\DimEdge}%
   {\ChgEdgeLineStyle{\DimEdgeLineStyle}%
    \ChgEdgeLineWidth{\DimEdgeLineCoef}%
    \ChgEdgeLineColor{\DimEdgeLineColor}%
    \ChgEdgeLabelColor{\DimEdgeLabelColor}}%
\newcommand{\SetDimEdgePmts}[4]%
   {\renewcommand{\DimEdgeLineStyle}{#1}%
    \renewcommand{\DimEdgeLineCoef}{#2}%
    \renewcommand{\DimEdgeLineColor}{#3}%
    \renewcommand{\DimEdgeLabelColor}{#4}
    \renewcommand{\DimEdge}%
      {\ChgEdgeLineStyle{\DimEdgeLineStyle}%
       \ChgEdgeLineWidth{\DimEdgeLineCoef}%
       \ChgEdgeLineColor{\DimEdgeLineColor}%
       \ChgEdgeLabelColor{\DimEdgeLabelColor}}%
    }%
\newcommand{\UnDimEdge}%
   {\RstEdgeLineStyle%
    \RstEdgeLineWidth%
    \RstEdgeLineColor%
    \RstEdgeLabelColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% \section{Transition styles}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpsstyle{VCEdgeStyle}%
    {%
     linewidth=\EdgeLineWid,%
     linestyle=\EdgeLineSty,%
     linecolor=\EdgeLineCol,%
     bordercolor=\EdgeLineBorderColor,%
     border=\EdgeLineBorderWD,%
     fillstyle=none,% ???
     doubleline=false,%
%
     arrows=\EdgeArrowSty,%
     arrowsize=\EdgArrowWidthDim,%
     arrowlength=\EdgArrowLengthCoef,%
     arrowinset=\EdgArrowInsetCoef,%
%
     offset=\EdgeOff,%
     labelsep=\TransLabelSP,%
     nodesep=\NodeSP}%
\newpsstyle{VCDblEdgeStyle}% 
    {doubleline=true,%
     linewidth=\DblEdgLineCoef\EdgeLineWid,%
     doublesep=\DblEdgLineSep\EdgeLineWid,%
     doublecolor=\DblEdgLineColor,%
%
     arrowsize=\DblEdgArrowWidthDim,%
     arrowlength=\DblEdgArrowLengthCoef,%
     arrowinset=\DblEdgArrowInsetCoef}
%
\newpsstyle{VCBoxedEdgeLblStyle}%
    {%
     framesep=\BxdEdgLblSep pt,%
     fillstyle=solid,%
     fillcolor=\BxdEdgLblBkg,% 
     linewidth=\BxdEdgLblWdt pt,%
     linestyle=\BxdEdgLblStl,%
     linecolor=\BxdEdgLblCol,%
     doubleline=\BxdEdgLblDbl,%
     cornersize=relative,%
     framearc=\BxdEdgLblRnd}
%%%
\newcommand{\EdgeStyle}%
   {\psset{style=VCEdgeStyle}%
    \ifDblEdgLine\psset{style=VCDblEdgeStyle}\fi}
\newcommand{\BoxedEdgeLabelStyle}%
   {\psset{style=VCBoxedEdgeLblStyle}}
%%%%%\section{Edge label composition}%%%%%

% \makeatletter
% 
% \def\psRot#1(#2,#3){\***@makebox{\***@Rot#1(#2,#3)}}
% \def\***@Rot#1(#2,#3){%
% \pssetxlength\***@dima{#2}%
% \pssetylength\***@dimb{#3}%
% \leavevmode
% \***@Verb{%
% /xRot \***@number\***@dima\space def
% /yRot \***@number\***@dimb\space def}%
% \hbox{%
% \***@Verb{%
% /cosA #1 cos def
% /sinA #1 sin def
% /ax cosA def
% /by sinA def
% /cx sinA neg def
% /dy cosA def
% /ex xRot cosA mul neg xRot add yRot sinA mul add def
% /fy xRot sinA mul neg yRot add yRot cosA mul sub def
% {[ax by cx dy ex fy] concat
% } \***@TMChange}%
% \box\***@hbox%
% \***@Verb{\***@TMRestore}}}
% 
% \makeatother

\newcommand{\ComposedEdgLbl}[1]%
   {\textcolor{\EdgeLabelCol}%    
      {\scalebox{\EdgeLabelSca}%
         {\scalebox{\EdgeLabelScale}%
            {\EdgeLabelSz 
             \EdgLblMode\EdgeLabelSty{\VCLbl{#1}}\EdgLblMode}}}}%

\newcommand{\VCEdgeLabel}[1]%
    {\ifVCRigidEdgeLabel%
        {\textcolor{\EdgeLabelCol}%
           {\scalebox{\EdgeLabelSca}%
              {\scalebox{\EdgeLabelScale}%
                 {%
%                   \qdisk(0,0){2pt}
                 \Put*[rot={0*}](0,0)%
                    {\EdgeLabelSz%
                     \EdgLblMode\EdgeLabelSty{\VCLbl{#1}}\EdgLblMode}}}}}%
     \else% 
        {\textcolor{\EdgeLabelCol}%
           {\scalebox{\EdgeLabelSca}%
              {\scalebox{\EdgeLabelScale}%
                 {%
%                  \rput{0}(0,0)%
%                 \qdisk(0,0){2pt}%
                    {\EdgeLabelSz%
                     \EdgLblMode\EdgeLabelSty{\VCLbl{#1}}\EdgLblMode}}}}}%
     \fi}%

\newcommand{\naputnrotParam}{\ifVCRigidEdgeLabel N\else 0\fi}
% \newcommand{\mynrot}{\makeatletter\psk@rot\makeatother}
\newcommand{\WRLLbl}[2]%
    {\ifVCBoxedEdgeLabel%
        \BoxedEdgeLabelStyle
        \naput[npos=#1]{\psframebox{\VCEdgeLabel{#2}}}%
     \else%
        \naput*[npos=#1,ref=t,nrot=\naputnrotParam]{\VCEdgeLabel{#2}}%
     \fi}%
\newcommand{\WRRLbl}[2]%
    {\ifVCBoxedEdgeLabel%
        \BoxedEdgeLabelStyle
        \nbput[npos=#1]{\psframebox{\VCEdgeLabel{#2}}}%
     \else%
        \nbput*[npos=#1,ref=ur,nrot=\naputnrotParam]{\VCEdgeLabel{#2}}%
     \fi}%
\newcommand{\WRCLbl}[2]%
    {\ifVCBoxedEdgeLabel%
        \BoxedEdgeLabelStyle
        \ncput[npos=#1]{\psframebox{\VCEdgeLabel{#2}}}%
     \else%
        \ncput[npos=#1,nrot=\naputnrotParam]{\VCEdgeLabel{#2}}%
     \fi}%
% \newcommand{\WRLLbl}[2]%
%     {%
%      \ifVCRigidEdgeLabel%
%      \else%
%         \ifVCBoxedEdgeLabel%
% 	   \BoxedEdgeLabelStyle
% 	   \naput[npos=#1]{\psframebox{\ComposedEdgLbl{#2}}}%
% 	\else%
% 	   \naput[npos=#1]{\ComposedEdgLbl{#2}}%
% 	\fi%
%      \fi}
% \newcommand{\WRRLbl}[2]%
%     {%
%      \ifVCRigidEdgeLabel%
%      \else%
%         \ifVCBoxedEdgeLabel%
%            \BoxedEdgeLabelStyle
% 	   \nbput[npos=#1]{\psframebox{\ComposedEdgLbl{#2}}}%
% 	\else%
% 	   \nbput[npos=#1]{\ComposedEdgLbl{#2}}%
% 	\fi%
%      \fi}
% \newcommand{\WRCLbl}[2]%
%     {%
%      \ifVCRigidEdgeLabel%
%      \else%
%         \ifVCBoxedEdgeLabel%
% 	   \BoxedEdgeLabelStyle
% 	   \ncput[npos=#1]{\psframebox{\ComposedEdgLbl{#2}}}%
% 	\else%
% 	   \ncput[npos=#1]{\ComposedEdgLbl{#2}}%
% 	\fi%
%      \fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  \section{Edge drawing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\EdgeL}[4][{\EdgLblPos}]% 
   {\EdgeStyle\ncline{#2}{#3}\WRLLbl{#1}{#4}}
\newcommand{\EdgeR}[4][{\EdgLblPos}]%
   {\EdgeStyle \ncline{#2}{#3}\WRRLbl{#1}{#4}}
\newcommand{\EdgeC}[4][{\EdgLblPos}]%
   {\EdgeStyle \ncline{#2}{#3}\WRCLbl{#1}{#4}}
\newcommand{\Edge}[2]{\EdgeStyle \ncline{#1}{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% line
% label
% \newcommand{\EdgeLabelColor}{black}
% \newcommand{\EdgeLabelScale}{1.7}
% %%% Dimmed edges 
% \newcommand{\DimEdgeLineCoef}{1.2} 
% \newcommand{\DimEdgeLineStyle}{solid} 
% \newcommand{\DimEdgeLineColor}{gray}
% \newcommand{\DimEdgeLabelColor}{gray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  \section{Zigzag edges}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Zigzag edges parameter
\newlength{\ZZSize}
\setlength{\ZZSize}{.9cm}%\MediumStateDiameter
\newcommand{\ZZShape}{0.5}
\newcommand{\ZZLineWidth}{1.7}% coefficient multiplicateur
\newcommand{\TransLabelZZCoef}{0.6}% coefficient multiplicateur
\newlength{\ZZSiZ}
\setlength{\ZZSiZ}{\ZZSize}%
\newcommand{\ZZLineWid}{\ZZLineWidth}% coefficient multiplicateur
% \newcommand{\ZZLineWid}{\ZZLineWidth}% coefficient multiplicateur
%
%%% zig-zag style
\newpsstyle{VCZZStyle}%
    {linewidth=\ZZLineWid\EdgeLineWid,%
     linearc=1.6pt,%
     coilwidth=1.2\ZZSiZ,%
     coilheight=\ZZShape,%
     coilarmA=0.1\ZZSiZ,%
     coilarmB=0.3\ZZSiZ,%
     labelsep=\TransLabelSP}
\newcommand{\ZZStyle}%
   {\addtolength{\TransLabelSP}{\TransLabelZZCoef\ZZSiZ}%
    \psset{style=VCZZStyle}%
    \addtolength{\TransLabelSP}{-\TransLabelZZCoef\ZZSiZ}}
%%% Zigzag edges
\newcommand{\ZZEdge}[2]%
   {\EdgeStyle\ZZStyle\nczigzag{#1}{#2}}
\newcommand{\ZZEdgeL}[4][{\EdgLblPos}]%
   {\EdgeStyle\ZZStyle\nczigzag{#2}{#3}\WRLLbl{#1}{#4}}
\newcommand{\ZZEdgeR}[4][{\EdgLblPos}]%
   {\EdgeStyle\ZZStyle\nczigzag{#2}{#3}\WRRLbl{#1}{#4}}
\newcommand{\ZZEdgeC}[4][{\EdgLblPos}]%
   {\EdgeStyle\ZZStyle\nczigzag{#2}{#3}\WRCLbl{#1}{#4}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% flags 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge geometric parameters  --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Edge label parameters --- Initial settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% label distance from transition
% \newlength{\TransLabelSP}\setlength{\TransLabelSP}{\TransLabelSep}
% label position on transitions
% \newcommand{\EdgeLabelPos}{\EdgeLabelPosit}
% \newcommand{\ArcLabelPos}{\ArcLabelPosit}
% \newcommand{\LArcLabelPos}{\LArcLabelPosit}
% \newcommand{\LoopLabelPos}{\LoopLabelPosit}
% \newcommand{\CLoopLabelPos}{\CLoopLabelPosit}
% label position on initial-final arrow
\newcommand{\InitStateLabelPos}{\InitStateLabelPosit}
\newcommand{\FinalStateLabelPos}{\FinalStateLabelPosit}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Transition styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%
% \newcommand{\ChgZZSize}[1]{\setlength{\ZZSiZ}{#1}}
% \newcommand{\RstZZSize}{\setlength{\ZZSiZ}{\ZZSize}}
% \newcommand{\SetZZSize}[1]{\setlength{\ZZSiZe}{#1}\RstZZSize}
% %%%\ZZLineWidth
% \newcommand{\ChgZZLineWidth}[1]{\renewcommand{\ZZLineWid}{#1}}
% \newcommand{\RstZZLineWidth}{\ChgZZLineWidth{\ZZLineWidth}}
% \newcommand{\SetZZLineWidth}[1]%
%    {\renewcommand{\ZZLineWidth}{#1}\RstZZLineWidth}
% %
%%% label of transitions
\newcommand{\VaucEdgeLabel}[1]{%
        \textcolor{\EdgeLabelCol}{\scalebox{\EdgeLabelSca}{\scalebox{\EdgeLabelScale}{$ #1 $}}}}
%%%
\newcommand{\RstEdge}{%
   \RstEdgeOffset\RstArcAngle\RstLArcAngle%
   \RstArcCurvature\RstLArcCurvature%
   \RstArcOffset\RstLoopOffset\RstLoopSize%
   \RstEdgeLineColor\RstEdgeLineStyle\RstEdgeLineWidth\EdgeLineSimple%
   \StraightArrow%\EdgeBorderOff%
   \RstEdgeLabelScale\RstEdgeLabelColor}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% implicit parameter
\newcommand{\InitialDir}{}\newcommand{\FinalDir}{}
\newcommand{\Dirnum}{}
%%% Size of initial and final arrow
% the size is relative to the diameter
% and the coefficient varies with the diameter
\newcommand{\ArrowOnStateCoef}{}
\newcommand{\ArrowOnMediumState}{}
\newcommand{\ArrowOnSmallState}{} 
\newcommand{\ArrowOnLargeState}{}
% ??? 120514
\newlength{\IFArwLgt}%
\newcommand{\SetIFArwLgt}{\setlength{\IFArwLgt}{\ArrowOnStateCoef\StateDia}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compute the distance for initial and final arrows
\newlength{\IFSDst}%
\newcommand{\CptIFSDst}%
   {%
    \setlength{\IFArwLgt}{\ArrowOnStateCoef\StateDia}%
    \VCSGGreaterLgt{\LastSttDrawnWidth}{\LastSttDrawnHeight}{\VCSGTmpLength}%
    \CorrPosSttIntDim{\VCSGTmpLength}%
    \setlength{\IFSDst}{.5\VCSGTmpLength}%
    \addtolength{\IFSDst}{\IFArwLgt}%
    }
% set the end point of initial and final arrows
\newcommand{\SetIFSNode}[2]%
   {%
    \VCSGCompassDecode{#1}{\Dirnum}%
    \CptIFSDst%
    \SpecialCoor%
    \uput{\IFSDst}[\Dirnum](#2){\pnode{#2qif}}%
    \NormalCoor%
    }
% without label new version 1205014
\newcommand{\Initial}[2][\InitialDir]%
   {\SetIFSNode{#1}{#2}%
    \EdgeStyle\ncline{#2qif}{#2}}
\newcommand{\Final}[2][\FinalDir]%
   {\SetIFSNode{#1}{#2}%
    \EdgeStyle\ncline{#2}{#2qif}}
% with label new version 1205014
%  NB modified syntax eg \InitialL[pos]{dir}{statename}{label}
\newcommand{\InitialL}[4][{\InitStateLabelPos}]%
   {\SetIFSNode{#2}{#3}%
    \EdgeStyle\ncline{#3qif}{#3}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\InitialR}[4][{\InitStateLabelPos}]%
   {\SetIFSNode{#2}{#3}%
    \EdgeStyle\ncline{#3qif}{#3}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalL}[4][{\FinalStateLabelPos}]%
   {\SetIFSNode{#2}{#3}%
    \EdgeStyle\ncline{#3}{#3qif}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
\newcommand{\FinalR}[4][{\FinalStateLabelPos}]%
   {\SetIFSNode{#2}{#3}%
    \EdgeStyle\ncline{#3}{#3qif}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
% % without label old version
% \newcommand{\Initial}[2][\InitialDir]%
%    {\VCSGCompassDecode{#1}{\Dirnum}%
%     \CptIFSDst%
%     \SpecialCoor%
%     \uput{\IFSDst}[\Dirnum](#2){\pnode{qz}}%
%     \NormalCoor%
%     \EdgeStyle\ncline{qz}{#2}}
% \newcommand{\Final}[2][\FinalDir]%
%    {\VCSGCompassDecode{#1}{\Dirnum}%
%     \CptIFSDst%
%     \SpecialCoor%
%     \uput{\IFSDst}[\Dirnum](#2){\pnode{qz}}%
%     \NormalCoor%
%     \EdgeStyle\ncline{#2}{qz}}
% % with label
% %  NB modified syntax eg \InitialL[pos]{dir}{statename}{label}
% \newcommand{\InitialL}[4][{\InitStateLabelPos}]%
%    {\EdgeStyle\ncline{#3#2}{#3}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
% \newcommand{\InitialR}[4][{\InitStateLabelPos}]%
%    {\EdgeStyle\ncline{#3#2}{#3}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
% \newcommand{\FinalL}[4][{\FinalStateLabelPos}]%
%    {\EdgeStyle\ncline{#3}{#3#2}\naput[npos=#1]{\VaucEdgeLabel{#4}}}
% \newcommand{\FinalR}[4][{\FinalStateLabelPos}]%
%    {\EdgeStyle\ncline{#3}{#3#2}\nbput[npos=#1]{\VaucEdgeLabel{#4}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Arc drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Arc parameters
% Angle
\newcommand{\ArcAngle}{}\newcommand{\ArcAng}{}
\newcommand{\LArcAngle}{}\newcommand{\LArcAng}{}
% Curvature
\newcommand{\ArcCurvature}{}\newcommand{\ArcCurv}{}
\newcommand{\LArcCurvature}{}\newcommand{\LArcCurv}{}
% Offset
\newlength{\ArcOffset}\newlength{\ArcOff}
%%% Arc parameter changing/setting
\newcommand{\ChgArcAngle}[1]{\renewcommand{\ArcAng}{#1}}
\newcommand{\RstArcAngle}{\ChgArcAngle{\ArcAngle}}
\newcommand{\SetArcAngle}[1]%
   {\renewcommand{\ArcAngle}{#1}\RstArcAngle}
%
\newcommand{\ChgLArcAngle}[1]{\renewcommand{\LArcAng}{#1}}
\newcommand{\RstLArcAngle}{\ChgLArcAngle{\LArcAngle}}
\newcommand{\SetLArcAngle}[1]%
   {\renewcommand{\LArcAngle}{#1}\RstLArcAngle}
%
\newcommand{\ChgArcCurvature}[1]{\renewcommand{\ArcCurv}{#1}}
\newcommand{\RstArcCurvature}{\ChgArcCurvature{\ArcCurvature}}
\newcommand{\SetArcCurvature}[1]%
   {\renewcommand{\ArcCurvature}{#1}\RstArcCurvature}
%
\newcommand{\ChgLArcCurvature}[1]{\renewcommand{\LArcCurv}{#1}}
\newcommand{\RstLArcCurvature}{\ChgLArcCurvature{\LArcCurvature}}
\newcommand{\SetLArcCurvature}[1]%
   {\renewcommand{\LArcCurvature}{#1}\RstLArcCurvature}
%
\newcommand{\ChgArcOffset}[1]{\setlength{\ArcOff}{#1}}
\newcommand{\RstArcOffset}{\setlength{\ArcOff}{\ArcOffset}}
\newcommand{\SetArcOffset}[1]%
   {\renewcommand{\ArcOffset}{#1}\RstArcOffset}
%%% Arc drawing styles
\newcommand{\ArcLStyle}%
    {\psset{ncurv=\ArcCurv,arcangle=\ArcAng,offset=\ArcOff}}
\newcommand{\ArcRStyle}%
    {\psset{ncurv=\ArcCurv,arcangle=-\ArcAng,offset=-\ArcOff}}
\newcommand{\LArcLStyle}%
    {\psset{ncurv=\LArcCurv,arcangle=\LArcAng,offset=\ArcOff}}
\newcommand{\LArcRStyle}%
    {\psset{ncurv=\LArcCurv,arcangle=-\LArcAng,offset=-\ArcOff}}
%%% Arc drawing commands
\newcommand{\ArcL}[4][{\ArcLblPos}]%
   {\EdgeStyle \ArcLStyle \ncarc{#2}{#3} \WRLLbl{#1}{#4}}%\naput[npos=#1]{\VCEdgeLabel{#4}}
\newcommand{\ArcR}[4][{\ArcLblPos}]%
   {\EdgeStyle \ArcRStyle \ncarc{#2}{#3} \WRRLbl{#1}{#4}}%
\newcommand{\LArcL}[4][{\LArcLblPos}]%
   {\EdgeStyle \LArcLStyle \ncarc{#2}{#3} \WRLLbl{#1}{#4}}%
\newcommand{\LArcR}[4][{\LArcLblPos}]%
   {\EdgeStyle \LArcRStyle \ncarc{#2}{#3} \WRRLbl{#1}{#4}}%
\newcommand{\ArcLC}[4][{\ArcLblPos}]%
   {\EdgeStyle \ArcLStyle \ncarc{#2}{#3} \WRCLbl{#1}{#4}}%\naput[npos=#1]{\VCEdgeLabel{#4}}
\newcommand{\ArcRC}[4][{\ArcLblPos}]%
   {\EdgeStyle \ArcRStyle \ncarc{#2}{#3} \WRCLbl{#1}{#4}}%
\newcommand{\LArcLC}[4][{\LArcLblPos}]%
   {\EdgeStyle \LArcLStyle \ncarc{#2}{#3} \WRCLbl{#1}{#4}}%
\newcommand{\LArcRC}[4][{\LArcLblPos}]%
   {\EdgeStyle \LArcRStyle \ncarc{#2}{#3} \WRCLbl{#1}{#4}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Loop drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Loop parameters
% Angle
\newcommand{\LoopAngle}{}\newcommand{\LoopAng}{}
\newcommand{\CLoopAngle}{}\newcommand{\CLoopAng}{}
% Size
\newcommand{\LoopSize}{}\newcommand{\LoopSi}{}
\newcommand{\CLoopSize}{}\newcommand{\CLoopSi}{}
% Offset
\newlength{\LoopOffset}\newlength{\LoopOff}
% Preset sizes of loops (depending on the size of the state)
\newcommand{\LoopOnSmallState}{} 
\newcommand{\LoopOnMediumState}{}
\newcommand{\LoopOnLargeState}{} 
%
\newcommand{\CLoopOnSmallState}{}
\newcommand{\CLoopOnMediumState}{}
\newcommand{\CLoopOnLargeState}{}
%%% Loop parameters% Size
%
\newcommand{\ChgLoopSize}[1]{\renewcommand{\LoopSi}{#1}}
\newcommand{\RstLoopSize}{\ChgLoopSize{\LoopSize}}
\newcommand{\SetLoopSize}[1]%
   {\renewcommand{\LoopSize}{#1}\RstLoopSize}
%
\newcommand{\ChgCLoopSize}[1]{\renewcommand{\CLoopSi}{#1}}
\newcommand{\RstCLoopSize}{\ChgCLoopSize{\CLoopSize}}
\newcommand{\SetCLoopSize}[1]%
   {\renewcommand{\CLoopSize}{#1}\RstCLoopSize}
% Angle
\newcommand{\ChgLoopAngle}[1]{\renewcommand{\LoopAng}{#1}}
\newcommand{\RstLoopAngle}{\ChgLoopAngle{\LoopAngle}}
\newcommand{\SetLoopAngle}[1]%
   {\renewcommand{\LoopAngle}{#1}\RstLoopAngle}
%
\newcommand{\ChgCLoopAngle}[1]{\renewcommand{\CLoopAng}{#1}}
\newcommand{\RstCLoopAngle}{\ChgCLoopAngle{\CLoopAngle}}
\newcommand{\SetCLoopAngle}[1]%
   {\renewcommand{\CLoopAngle}{#1}\RstCLoopAngle}
% Offset
\newcommand{\ChgLoopOffset}[1]{\setlength{\LoopOff}{#1}}
\newcommand{\RstLoopOffset}{\setlength{\LoopOff}{\LoopOffset}}
\newcommand{\SetLoopOffset}[1]%
   {\renewcommand{\LoopOffset}{#1}\RstLoopOffset}
%
%%%%
\newcounter{anglea}\newcounter{angleb}
\newcommand{\LoopXR}[7]%
   {{\setcounter{anglea}{#2-#4}}%
    {\setcounter{angleb}{#2+#4}}%
    {\EdgeStyle \psset{angleA=\theanglea,angleB=\theangleb,offset=#5,ncurv=#6}% 
    \nccurve{#3}{#3} \WRRLbl{#1}{#7}}}%\nbput[npos=#1]{\VaucEdgeLabel{#7}}
\newcommand{\LoopXL}[7]%
   {{\setcounter{anglea}{#2+#4}}%
    {\setcounter{angleb}{#2-#4}}%
    {\EdgeStyle \psset{angleA=\theanglea,angleB=\theangleb,offset=-#5,ncurv=#6}% 
    \nccurve{#3}{#3} \WRLLbl{#1}{#7}}}%\naput[npos=#1]{\VaucEdgeLabel{#7}}
\newcommand{\LoopR}[4][{\LoopLblPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopL}[4][{\LoopLblPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopR}[4][{\CLoopLblPos}]%
   {\LoopXR{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\CLoopL}[4][{\CLoopLblPos}]%
   {\LoopXL{#1}{#2}{#3}{\CLoopAng}{\LoopOff}{\LoopSi}{#4}}
\newcommand{\LoopVarR}[4][{\LoopLblPos}]%
   {\LoopXR{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopVarL}[4][{\LoopLblPos}]%
   {\LoopXL{#1}{#2}{#3}{\LoopVarAng}{\LoopVarOff}{\LoopVarSi}{#4}}
\newcommand{\LoopW}[3][{\LoopLblPos}]{\LoopR[#1]{180}{#2}{#3}}
\newcommand{\LoopE}[3][{\LoopLblPos}]{\LoopL[#1]{0}{#2}{#3}}
\newcommand{\LoopN}[3][{\LoopLblPos}]{\LoopL[#1]{90}{#2}{#3}}
\newcommand{\LoopS}[3][{\LoopLblPos}]{\LoopR[#1]{-90}{#2}{#3}}
\newcommand{\LoopNW}[3][{\LoopLblPos}]{\LoopR[#1]{135}{#2}{#3}}
\newcommand{\LoopNE}[3][{\LoopLblPos}]{\LoopL[#1]{45}{#2}{#3}}
\newcommand{\LoopSW}[3][{\LoopLblPos}]{\LoopL[#1]{-135}{#2}{#3}}
\newcommand{\LoopSE}[3][{\LoopLblPos}]{\LoopR[#1]{-45}{#2}{#3}}
\newcommand{\CLoopW}[3][{\CLoopLblPos}]{\CLoopR[#1]{180}{#2}{#3}}
\newcommand{\CLoopE}[3][{\CLoopLblPos}]{\CLoopL[#1]{0}{#2}{#3}}
\newcommand{\CLoopN}[3][{\CLoopLblPos}]{\CLoopL[#1]{90}{#2}{#3}}
\newcommand{\CLoopS}[3][{\CLoopLblPos}]{\CLoopR[#1]{-90}{#2}{#3}}
\newcommand{\CLoopNW}[3][{\CLoopLblPos}]{\CLoopR[#1]{135}{#2}{#3}}
\newcommand{\CLoopNE}[3][{\CLoopLblPos}]{\CLoopL[#1]{45}{#2}{#3}}
\newcommand{\CLoopSW}[3][{\CLoopLblPos}]{\CLoopL[#1]{-135}{#2}{#3}}
\newcommand{\CLoopSE}[3][{\CLoopLblPos}]{\CLoopR[#1]{-45}{#2}{#3}}
\newcommand{\LoopVarN}[3][{\CLoopLblPos}]{\LoopVarL[#1]{90}{#2}{#3}}
\newcommand{\LoopVarS}[3][{\CLoopLblPos}]{\LoopVarR[#1]{-90}{#2}{#3}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ReverseArrow}{\ReverseTransitions}%
\newcommand{\StraightArrow}{\DirectTransitions}%
\newcommand{\FixDimEdge}[4]{\SetDimEdgePmts{#1}{#2}{#3}{#4}}%
\newcommand{\EdgeBorder}{\EdgeLineBorderOn}%
\newcommand{\EdgeBorderOff}{\EdgeLineBorderOff}%
\newcommand{\FixEdgeBorder}[2]{\FixEdgeLineBorder{#1}{#2}}%
\newcommand{\ForthBackOffset}{\ForthBackOffsetOn}%
%
\newcommand{\SetEdgeArrowWidth}[1]{\SetEdgeArrowWidthBase{#1}}			%width of the edge arrow
\newlength{\EdgeDblArrowWidth}		%width : 
\setlength{\EdgeDblArrowWidth}{1.3mm}		%width : 
\newcommand{\EdgeDblArrowLengthCoef}{}	% 
%
\newcommand{\EdgeLabelPosit}{}\newcommand{\EdgeLabelRevPosit}{}
\newcommand{\ArcLabelPosit}{}\newcommand{\ArcLabelRevPosit}{}
\newcommand{\LArcLabelPosit}{}\newcommand{\LArcLabelRevPosit}{}
\newcommand{\LoopLabelPosit}{}\newcommand{\LoopLabelRevPosit}{}
\newcommand{\CLoopLabelPosit}{}\newcommand{\CLoopLabelRevPosit}{}
%
\newcommand{\LoopVarAngle}{}\newcommand{\LoopVarAng}{}
\newcommand{\LoopVarSize}{}\newcommand{\LoopVarSi}{}
\newlength{\LoopVarOffset}\newlength{\LoopVarOff}
\newcommand{\LoopOnVariableState}{} 
\newcommand{\CLoopOnVariableState}{}
\newcommand{\LoopOnVerySmallState}{} 
%
\newcommand{\ChgLoopVarSize}[1]{\renewcommand{\LoopVarSi}{#1}}
\newcommand{\RstLoopVarSize}{\ChgLoopVarSize{\LoopVarSize}}
\newcommand{\SetLoopVarSize}[1]%
   {\renewcommand{\LoopVarSize}{#1}\RstLoopVarSize}
% label position on initial-final arrow
\newcommand{\InitStateLabelPosit}{}\newcommand{\InitStateLabelRevPosit}{}
\newcommand{\FinalStateLabelPosit}{}\newcommand{\FinalStateLabelRevPosit}{}
%
\newcommand{\ArrowOnVerySmallState}{5} 
%
\newcommand{\VArcL}[5][{\ArcLblPos}]%
   {\EdgeStyle \ArcLStyle%\psset{style=VaucLArcL} 
    \ncarc[#2]{#3}{#4} \WRLLbl{#1}{#5}}%\naput[npos=#1]{\VaucEdgeLabel{#5}}
\newcommand{\VArcR}[5][{\ArcLblPos}]%
   {\EdgeStyle \ArcRStyle%\psset{style=VaucLArcR} 
    \ncarc[#2]{#3}{#4} \WRRLbl{#1}{#5}}%\nbput[npos=#1]{\VaucEdgeLabel{#5}}
%
\newcommand{\VCurveL}[5][{\ArcLblPos}]%
   {\EdgeStyle \psset{angleA=0,angleB=180,ncurv=1}% 
    \nccurve[#2]{#3}{#4} \WRLLbl{#1}{#5}}%\naput[npos=#1]{\VaucEdgeLabel{#5}}
\newcommand{\VCurveR}[5][{\ArcLblPos}]%
   {\EdgeStyle \psset{angleA=0,angleB=0,ncurv=1}% 
    \nccurve[#2]{#3}{#4} \WRRLbl{#1}{#5}}%\nbput[npos=#1]{\VaucEdgeLabel{#5}}
%
\newcommand{\LabelL}[2][{\EdgLblPos}]{\WRLLbl{#1}{#2}}%\naput[npos=#1]{\VaucEdgeLabel{#2}}
\newcommand{\LabelR}[2][{\EdgLblPos}]{\WRRLbl{#1}{#2}}%\nbput[npos=#1]{\VaucEdgeLabel{#2}}
%%%  Initial-final quality: obsolete as the phantom positions are not 
%%%  generated anymore
\newcommand{\VCIFflag}{2}\newcommand{\VCIFflagtemp}{2}
\newcommand{\PlainState}{}%
\newcommand{\FullState}{}%
\newcommand{\IFState}{}
\newcommand{\IFXState}{}
\newcommand{\RstVCIF}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
arrows=\EdgeArrowSty,%
arrowsize=\EdgArrowWidthDim,%
arrowlength=\EdgArrowLengthCoef,%
arrowinset=\EdgArrowInsetCoef,%
\newcommand{\SetEdgArrowWD}% internal function
   {\setlength{\EdgArrowWidthDim}{\EdgArrowWDBase}%
    \addtolength{\EdgArrowWidthDim}{\EdgArrowWidthCoef\EdgeLineWid}}
\newcommand{\SetDblEdgArrowWD}% internal function
   {\setlength{\DblEdgArrowWidthDim}{\DblEdgArrowWDBase}%
    \addtolength{\DblEdgArrowWidthDim}%
                {\DblEdgArrowWidthCoef\DblEdgLineWD}}


==> VCSG-environment.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-environment
%%
%% DESCRIPTION:  Definition of the picture environment
%%
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%    2.1 - 050219
%    2.2 - 050727
%    2.3 - 060628     Modif. induced by VCSG-edgess
%          091016     \VCInputFig added
%          091028     Calls for version compatibility and 
%                     initialisation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Scaling matters}%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% "Sizes" (eg for states) and "widths" (of lines) are given 
%%% as "lengthes" in a fixed unit (cm or pt), 
%%% whereas the positions are normally given in "psunits".
%%% 
%%% This allows to use different scaling parameters 
%%% for the whole figure and for the "drawing grid".
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scaling parameters
\newcommand{\VCScale}{}%      Global scale parameter
\newcommand{\VCGridScale}{}%  Grid scale parameter
\newcommand{\LargeScale}{}%   Preset value
\newcommand{\MediumScale}{}%  Preset value
\newcommand{\SmallScale}{}%   Preset value
\newcommand{\TinyScale}{}%    Preset value
\newcommand{\LargeScaleI}{}%   Preset value
\newcommand{\MediumScaleI}{}%  Preset value
\newcommand{\SmallScaleI}{}%   Preset value
\newcommand{\TinyScaleI}{}%    Preset value
%%% Scaling commands
% general
\newcommand{\FixVCScale}[1]{\renewcommand{\VCScale}{#1}}% 
\newcommand{\FixVCGridScale}[1]{\renewcommand{\VCGridScale}{#1}}%
\newcommand{\FixPctScale}[2]%
   {\renewcommand{\VCScale}{#1}%
    \SetStateLabelScale{#2}%
    \SetEdgeLabelScale{#2}%
    \FixVCGridScale{1}%
   }% 
% with preset parameters
\newcommand{\LargePictures}{\FixPctScale{\LargeScale}{\LargeScaleI}}
\newcommand{\MediumPictures}{\FixPctScale{\MediumScale}{\MediumScaleI}}
\newcommand{\SmallPictures}{\FixPctScale{\SmallScale}{\SmallScaleI}}
\newcommand{\TinyPictures}{\FixPctScale{\TinyScale}{\TinyScaleI}}
% for compatibility
\newcommand{\LargePicture}{\FixVCScale{\LargeScale}\FixVCGridScale{1}}
\newcommand{\MediumPicture}{\FixVCScale{\MediumScale}\FixVCGridScale{1}}
\newcommand{\SmallPicture}{\FixVCScale{\SmallScale}\FixVCGridScale{1}}
\newcommand{\TinyPicture}{\FixVCScale{\TinyScale}\FixVCGridScale{1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Picture directory}%%%%%
\newcommand{\VCDirectory}{}% the definition is an initialisation
\newcommand{\SetVCDirectory}[1]{\renewcommand{\VCDirectory}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Picture framing}%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% flags 
\newif\ifVCFrame% showing/hiding the frame "around" the picture
\newcommand{\HideFrame}{\VCFramefalse}
\newcommand{\ShowFrame}{\VCFrametrue}
\newif\ifVCGrid% showing/hiding the grid in the frame
\newcommand{\HideGrid}{\VCGridfalse}
\newcommand{\ShowGrid}%
   {\VCGridtrue%
    \renewcommand{\VCGridLabelColor}{\VCGridLineColor}}
\newcommand{\ShowGridNL}%
   {\VCGridtrue%
    \renewcommand{\VCGridLabelColor}{white}}
\newif\ifVCName% printing/or not the name of the figure file
\newcommand{\HideName}{\VCNamefalse}
\newcommand{\ShowName}{\VCNametrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  inner parameters (no doubling)
\newcommand{\VCBkgdStyle}{}
\newcommand{\VCBkgdColor}{}
\newcommand{\SetVCBkgdStyle}[1]%% ATTN Reset Bkgd for states
    {\renewcommand{\VCBkgdStyle}{#1}%
     \SetStateBkgdStyle{#1}}
\newcommand{\SetVCBkgdColor}[1]%% ATTN Reset Bkgd for states
    {\renewcommand{\VCBkgdColor}{#1}%
     \SetStateBkgdColor{#1}%
     \renewcommand{\SttBorderColor}{#1}% Border -- see VCSG-states
     \SetEdgeLineBorderColor{#1}% Border -- see VCSG-edges
     \SetDblEdgeLineColor{#1}% double lines -- see VCSG-edges
    }%
% (to be changed with a \renewcommand)
\newlength{\VCFrameLineWidth}{}
\newcommand{\VCFrameLineColor}{}
\newlength{\VCGridLineWidth}{}
\newcommand{\VCGridLineColor}{}
\newcommand{\VCGridLabelColor}{}% in view of \ShowGridNL
\newcommand{\VCSubGridLineColor}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   styles for the background, frame and grid 
\newpsstyle{VCBkgdStyle}%
           {framesep=0pt,
            arrows=-,%                   
            linestyle=none,%
            linewidth=0.1pt,
            linecolor=black,%
            doubleline=false,%
            dimen=inner,% the frame has exactly the given size
            fillcolor=\VCBkgdColor,%
            fillstyle=\VCBkgdStyle,%
            griddots=0,% no grid a priori
            cornersize=relative,%
            framearc=0}
\newpsstyle{VCFrameStyle}% to be used just after VCBkgdStyle
           {linestyle=solid,%
            linewidth=\VCFrameLineWidth,%
	    linecolor=\VCFrameLineColor,%
            doubleline=false}%,
\newpsstyle{VCGridStyle}% to be used just after VCFrameStyle
           {gridwidth=\VCGridLineWidth,%
            griddots=10,%
	    gridcolor=\VCGridLineColor,%
            gridlabels=7pt,%
            gridlabelcolor=\VCGridLabelColor,%
            subgridwidth=0.2pt,%
            subgriddiv=5,%
            subgridcolor=\VCSubGridLineColor}
\newcommand{\BkgdStyle}{\psset{style=VCBkgdStyle}}
\newcommand{\FrameStyle}{\psset{style=VCFrameStyle}}
\newcommand{\GridStyle}%
   {\ifthenelse{\equal{\VCGridLineColor}{black}}% 
       {\renewcommand{\VCSubGridLineColor}{black}}%
       {\renewcommand{\VCSubGridLineColor}{\VCGridLineColor}}%
    \psset{style=VCGridStyle}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Picture drawing call}%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In order to make the parameter VCScale part of the environment and 
% dealt with by VauCanSon-G commands, the call look like:
%
%  \VCDraw{%
%     \begin{VCPicture}{(x0,y0)(x1,y1)}
%     %  figure description ...
%     \end{VCPicture}%
%    }
%
% or like
%
% \VCCall{figure-file-name}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  parameters
\newlength{\VCSGMinHeight}%
\newlength{\VCSGMaxHeight}%
\newcommand{\VCVertPlac}{}%
\newcommand{\FixVerticalPlacement}[1]{\renewcommand{\VCVertPlac}{#1}}
%%%  picture environment
\newenvironment{VCPicture}[2][\VCVertPlac]%
  {%
   \pssetlength{\VCSGMinHeight}{\VCSGProjectionOnSecondComponent#2}%
   \pssetlength{\VCSGMaxHeight}{\VCSGProjectionOnFourthComponent#2}%
   \addtolength{\VCSGMinHeight}{-\VCSGMaxHeight}%
   \begin{pspicture}[shift=#1\VCSGMinHeight]#2%
       \BkgdStyle \psframe#2%
       \ifVCFrame \FrameStyle \psframe#2\fi%
       \ifVCGrid  \FrameStyle \GridStyle \psgrid#2\fi}%
  {\RstState
% %     \RstVertex%
% %     \RstEdge%
   \end{pspicture}}%
%%%  calls to the picture environment
\newcommand{\VCDraw}[2][\VCGridScale]%
   {\psset{unit=#1cm}%
    \scalebox{\VCScale}{#2}%
    \psset{unit=\VCGridScale cm}}
%
\newcommand{\VCCall}[2][\VCGridScale]%
   {\psset{unit=#1cm}%
    \ifVCName\makebox[0pt][r]{\fbox{{\scriptsize #2}}}\fi%
    \scalebox{\VCScale}{\input{\VCDirectory #2}}%
    \psset{unit=\VCGridScale cm}}
%%%  call to part of a picture
% Allows to put parts of figures in the \VCDirectory 
% and to call them inside a \VCDraw
\newcommand{\VCInputFig}[1]{\input{\VCDirectory #1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{VauCanSon-G modes}%%%%%
\newcommand{\VCMode}{}  
\newcommand{\Automata}%
   {\renewcommand{\VCMode}{automata}\SizedNodes}
\newcommand{\Graphs}%
   {\renewcommand{\VCMode}{graphs}\SizelessNodes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Version compatibility}%%%%%
\newcommand{\VCSGZeroFour}{\input VCPref-version04.tex }
\newcommand{\VCSGOne}{\input VCPref-version1.tex }
\newcommand{\VCSGInit}{\input VCSG-Preferences.tex }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> VCSG-functions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-functions.tex
%%
%% DESCRIPTION:
%%
%%   Auxiliary functions and variables called inside VauCanSon-G 
%%   PSTricks commands to be used inside pictures with VauCanSon-G's 
%%   syntax 
%%  
%% DATE:    2008/12/28
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{constants}%%%%%%%%
\newcommand{\VCSG}
     {\textsc{V$\overline{\text{au}}$%
              C\raisebox{.3ex}{$\underline{\text{an}}$}%
              S$\overline{\text{on}}$-G}\xspace}
\newcommand{\vcsg}
     {\textsc{V$\overline{\text{cs}}$G}\xspace}
\newcommand{\Vaucanson}{\VCSG}% compatibility (with what??)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Constants for geometric constructions
\newcommand{\HSQRTwo}{0.717}
\newcommand{\SQRThree}{1.732}
\newcommand{\GoldMean}{0.618}
\newcommand{\GoldMeanI}{1.618}
\newcommand{\SQRGoldMeanI}{1.272}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% If it has to be somewhere before the preferences, here is the best
\psset{unit=1cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{constants}%%%%%%%%
\newlength{\VCSGTmpLength}
\newlength{\VCSGTmpLengthbis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{functions}%%%%%%%%
\def\VCSGProjectionOnSecondComponent(#1,#2)(#3,#4){#2}%
\def\VCSGProjectionOnFourthComponent(#1,#2)(#3,#4){#4}%
%%% Functions for dealing with numbers
\newcommand{\VCSGCmdPosTst}[1]{\lengthtest{#1pt > 0pt}}
\newcommand{\VCSGGreaterLgt}[3]%
    {\ifthenelse{\lengthtest{#1 > #2}\or\lengthtest{#1 = #2}}%
        {\setlength{#3}{#1}}%
        {\setlength{#3}{#2}}%
     }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Functions for geometric constructions
\newcommand{\VCSGCompassDecode}[2]%
% Translate the eight compass directions into degrees
% If #1 is not a compass direction, simply copy it into #2
   {\ifthenelse{\equal{#1}{n}}%#2
       {\renewcommand{#2}{90}}%
       {\ifthenelse{\equal{#1}{ne}}%
           {\renewcommand{#2}{45}}%
           {\ifthenelse{\equal{#1}{e}}%
               {\renewcommand{#2}{0}}%
               {\ifthenelse{\equal{#1}{se}}%
                   {\renewcommand{#2}{315}}%
                   {\ifthenelse{\equal{#1}{s}}%
                       {\renewcommand{#2}{270}}%
                       {\ifthenelse{\equal{#1}{sw}}%
                           {\renewcommand{#2}{225}}%
                           {\ifthenelse{\equal{#1}{w}}%
                               {\renewcommand{#2}{180}}%
                               {\ifthenelse{\equal{#1}{nw}}%
                                   {\renewcommand{#2}{135}}%
                                   {\renewcommand{#2}{#1}}}}}}}}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{PSTricks commands}
\newcommand{\Point}[2]{\pnode#1{#2}}
\newcommand{\VCPut}[3][0]{\rput{#1}#2{#3}}% 
\newcommand{\Translate}[2]{\rput#1{#2}}% 
\newcommand{\Rotate}[2]{\rput{#1}(0,0){#2}}% 
\newcommand{\TransRotate}[3]{\rput{#2}#1{#3}}% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
\newcommand{\SQRTwo}{0.717}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> VCSG-states.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCSG-states.tex
%%
%% DESCRIPTION:   Commands for drawing states
%%
%% DATE:    2009/01/06
%%
%% Copyright (C) 2009 Sylvain Lombardy and Jacques Sakarovitch
%    2.1 - 05/02/19
%    2.2 - 05/03/02    VCS-states
%    2.3 - 05/07/29    include VCS-state-labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Node mode}%%%%%%
%%% A flag to distinguish between "sized" and "sizeless" nodes
\newif\ifVCSizedNode   
\newcommand{\SizedNodes}{\VCSizedNodetrue}
\newcommand{\SizelessNodes}{\VCSizedNodefalse}
%%% synonymous
\newcommand{\SizedStates}{\SizedNodes}
\newcommand{\SizelessStates}{\SizelessNodes}
\newcommand{\SizedVertices}{\SizedNodes}
\newcommand{\SizelessVertices}{\SizelessNodes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state size}%%%%%%
%%%  A variable to remember the current size of states
\newcommand{\VCSttSize}{}
% VSState (very small state) does not change the value:
%                                 it is not a mode that is remembered
%  That variable allows to fix (via preset values) such parameters as
%  the lenght of initial or final arrows and 
%  the curvature and offset of loops 
%  No effect on Vertex
% %%% Size = StateSize
%%% mod. 2.3  change to a more logical terminology
%%% The `size' of a state is `small', `medium' or `large'
%%% The `diameter' of a state is a length.
\newlength{\StateDiameter}\newlength{\StateDia}
%%%   Preset size parameters
%%% The preset sizes are given in cm, and not in "psunits".
%%% This allows to use different scales for the whole figure 
%%% and for the "drawing grid".
\newlength{\MediumStateDiameter}
\newlength{\SmallStateDiameter}
\newlength{\LargeStateDiameter}
\newlength{\VerySmallStateDiameter}% may be to be moved
%%%
\newcommand{\FixStateSizes}[4]% 
   {\setlength{\SmallStateDiameter}{#1}%
    \setlength{\MediumStateDiameter}{#2}%
    \setlength{\LargeStateDiameter}{#3}%
    \setlength{\VerySmallStateDiameter}{#4}}
%%% Changes of the state diameter as it is commonly provided for other 
%%% parameters 
%%% is not recommanded for it should be accompanied by a modification
%%% of many other parameters (for the drawing of arcs and loops).
%%% and this is what the above commands are made for. ?????
%%% However it may be useful in some cases to be able to modify 
%%% the state diameter and we thus have the same set of commands as 
%%% for other parameters (the use of `Stt' instead of `State' is 
%%% supposed to be a reminder that they are almost
%%% internal commands.
\newcommand{\ChgSttDiameter}[1]{\setlength{\StateDia}{#1\StateDiameter}}  
\newcommand{\RstSttDiameter}{\ChgSttDiameter{1}}
\newcommand{\SetSttDiameter}[1]% 
   {\setlength{\StateDiameter}{#1}\RstSttDiameter}
\newcommand{\IncChgSttDiameter}[1]{\setlength{\StateDia}{#1\StateDia}}  
% 
\newcommand{\FixStateDiameter}[1]{\SetSttDiameter{#1}}  
%%% setting state size, and the other parameters that come along
\newcommand{\EstabSttSize}[5]%
   {%
    \renewcommand{\VCSttSize}{#1}%
    \SetSttDiameter{#2}%
    \renewcommand{\ArrowOnStateCoef}{#3}% en attendant la partie 
                                        % inital-final
    \SetLoopSize{#4}%         en attendant la partie edges
%     \SetLoopVarSize{#4}%
    \SetCLoopSize{#5}%
   }
%%%
\newcommand{\MediumStates}%
   {\EstabSttSize{medium}{\MediumStateDiameter}{\ArrowOnMediumState}%
	       {\LoopOnMediumState}{\CLoopOnMediumState}}
\newcommand{\SmallStates}%
   {\EstabSttSize{small}{\SmallStateDiameter}{\ArrowOnSmallState}%
               {\LoopOnSmallState}{\CLoopOnSmallState}}
\newcommand{\LargeStates}%
   {\EstabSttSize{large}{\LargeStateDiameter}{\ArrowOnLargeState}%
               {\LoopOnLargeState}{\CLoopOnLargeState}}
%%% recovering the current preset value for size
\newcommand{\RstStateSize}%
  {\ifthenelse{\equal{\VCSttSize}{medium}}%
              {\MediumStates}%
              {\ifthenelse{\equal{\VCSttSize}{small}}%
                          {\SmallStates}%
			  {\ifthenelse{\equal{\VCSttSize}{large}}%
			              {\LargeStates}{ErrStateSize}}}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state shape}%%%%%
%%%  A variable to remember the current shape of states
\newcommand{\VCSttShape}{}% remember the current shape of states
\newcommand{\VCSttShp}{}%   int. var. used when state is processed
% 
\newcommand{\CircleStates}{\renewcommand{\VCSttShape}{circle}}
\newcommand{\OvalStates}{\renewcommand{\VCSttShape}{oval}}
\newcommand{\SquareStates}{\renewcommand{\VCSttShape}{square}}
\newcommand{\RectangleStates}{\renewcommand{\VCSttShape}{rectangle}}
%%% shape of oval states
\newcommand{\OvalStateRatio}{}\newcommand{\OvalStateRat}{}
% changing/setting the shape of rectangular states
\newcommand{\ChgOvalStateRatio}[1]{\renewcommand{\OvalStateRat}{#1}}
\newcommand{\RstOvalStateRatio}%
   {\ChgOvalStateRatio{\OvalStateRatio}}
\newcommand{\SetOvalStateRatio}[1]%
   {\renewcommand{\OvalStateRatio}{#1}\RstOvalStateRatio}
%%% shape of rectangular states
\newcommand{\RectangleStateRatio}{}\newcommand{\RectangleStateRat}{}
% changing/setting the shape of rectangular states
\newcommand{\ChgRectangleStateRatio}[1]{\renewcommand{\RectangleStateRat}{#1}}
\newcommand{\RstRectangleStateRatio}%
   {\ChgRectangleStateRatio{\RectangleStateRatio}}
\newcommand{\SetRectangleStateRatio}[1]%
   {\renewcommand{\RectangleStateRatio}{#1}\RstRectangleStateRatio}
%%%  Rounding the corners of square/rectangular states
%  A flag to remember the rounding of square/rectangular states
\newif\ifRoundedState%
%%%  The rounding may be `relative' or `absolute'
%%%  Variables that follow record the mode of rounding and the 
%%%  corresponding parameters
\newcommand{\StateCornerRounding}{}% record the mode of rounding
% Setting the mode of rounding
\newcommand{\StateCornerRoundingAbsolute}%
   {\renewcommand{\StateCornerRounding}{absolute}}
\newcommand{\StateCornerRoundingRelative}%
   {\renewcommand{\StateCornerRounding}{relative}}
%  Relative rounding. Radius for rounded corners is a float
%                     Will be given in the psstyle as "framearc"
\newcommand{\StateCornerRelRadius}{}\newcommand{\StateCornerRelRad}{}
%   ATTN   Relative radius is "changed" "absolutely"
\newcommand{\ChgStateCornerRelRadius}[1]%
   {\renewcommand{\StateCornerRelRad}{#1}}
\newcommand{\RstStateCornerRelRadius}%
   {\ChgStateCornerRelRadius{\StateCornerRelRadius}}
\newcommand{\SetStateCornerRelRadius}[1]%
   {\renewcommand{\StateCornerRelRadius}{#1}\RstStateCornerRelRadius}
%  Absolute rounding. Radius for rounded corners is a length
%                     Will be given in the psstyle as "linearc"
%     Together with the usual 2 variables, xxxRadius and xxxRad, a 
%     third one, xxxRadEff, is the one that is given to the psstyle 
%     and allows to switch between sharp and rounded states without 
%     interfering wwith the normal process of rounded states
\newlength{\StateCornerRadius}\newlength{\StateCornerRad}
\newlength{\StateCornerRadEff}
%
\newcommand{\ChgStateCornerRadius}[1]%
   {\setlength{\StateCornerRad}{#1\StateCornerRadius}%
    \ifRoundedState\setlength{\StateCornerRadEff}{\StateCornerRad}\fi}
\newcommand{\RstStateCornerRadius}{\ChgStateCornerRadius{1}}
\newcommand{\SetStateCornerRadius}[1]%
   {\setlength{\StateCornerRadius}{#1}\RstStateCornerRadius}
% Switching between sharp and rounded corners
\newcommand{\SharpStateCorners}%
   {\RoundedStatefalse\setlength{\StateCornerRadEff}{0pt}}
\newcommand{\RoundedStateCorners}%
   {\RoundedStatetrue\setlength{\StateCornerRadEff}{\StateCornerRad}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Hiding -- showing}%%%%%
%%% Hiding -- showing states (used for overlays in slides)
% (used internally for the hidden states in adjusted states) 
% the trick is to have two different styles instead of 
% saving\restoring parameters
\newif\ifVCShowStt
\newcommand{\HideStates}{\VCShowSttfalse}
\newcommand{\ShowStates}{\VCShowStttrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state background parameters}%%%%%
\newcommand{\StateBkgdStyle}{}\newcommand{\StateBkgdSty}{} 
\newcommand{\StateBkgdColor}{}\newcommand{\StateBkgdCol}{}
   % As they have usually no labels it useful
   % to have a special coloring facility for the "SmallState"
   % especially for slide style
\newcommand{\SmallStateBkgdStyle}{}
\newcommand{\SmallStateBkgdColor}{} 
%%%  changing/setting macros
% changing/setting the background style 
\newcommand{\ChgStateBkgdStyle}[1]{\renewcommand{\StateBkgdSty}{#1}}
\newcommand{\RstStateBkgdStyle}{\ChgStateBkgdStyle{\StateBkgdStyle}}
\newcommand{\SetStateBkgdStyle}[1]% 
    {\renewcommand{\StateBkgdStyle}{#1}\RstStateBkgdStyle%
     \renewcommand{\SmallStateBkgdStyle}{#1}% ATTN reset Bkgd for 
                                            % Small States
    }
% changing/setting the background color 
\newcommand{\ChgStateBkgdColor}[1]{\renewcommand{\StateBkgdCol}{#1}}
\newcommand{\RstStateBkgdColor}{\ChgStateBkgdColor{\StateBkgdColor}}
\newcommand{\SetStateBkgdColor}[1]% 
    {\renewcommand{\StateBkgdColor}{#1}\RstStateBkgdColor%
     \renewcommand{\SmallStateBkgdColor}{#1}% ATTN reset Bkgd for 
                                            % Small States
    }
% setting SmallState background style and color 
\newcommand{\SetSmallStateBkgdStyle}[1]%
    {\renewcommand{\SmallStateBkgdStyle}{#1}}
\newcommand{\SetSmallStateBkgdColor}[1]%
    {\renewcommand{\SmallStateBkgdColor}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state line parameters}%%%%%%
\newlength{\StateLineWidth}\newlength{\StateLineWid}
% \newcommand{\VSStateLineCoef}{} % coef. for very small state
\newcommand{\StateLineStyle}{}\newcommand{\StateLineSty}{} 
\newcommand{\StateLineColor}{}\newcommand{\StateLineCol}{}
% parameters for double line
\newif\ifStateLineDbl 
\newcommand{\StateLineDbl}{} 
\newcommand{\SttLineDblCoef}{} 
\newcommand{\StateLineDblColor}{} 
\newcommand{\SttLineDblSep}{}\newcommand{\StateLineDblSp}{} 
% internal parameters
\newcommand{\SttDimen}{} 
\newcommand{\SttDblLineDimen}{}
% Border (of prescribed width and color) on both side of the line for 
% giving  the impression that one line passes above another. 
% May be useful when transitions cross over (under) states, but this 
% is not likely to happen so often.
\newlength{\SttBorderWidth}
\newcommand{\SttBorderColor}{}% normally same as state Bkgd
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  changing/setting macros 
% changing/setting the width of state line 
\newcommand{\ChgStateLineWidth}[1]%
   {\setlength{\StateLineWid}{#1\StateLineWidth}}  
\newcommand{\RstStateLineWidth}{\ChgStateLineWidth{1}}
\newcommand{\SetStateLineWidth}[1]% ATTN the parameter is a length
   {\setlength{\StateLineWidth}{#1}\RstStateLineWidth}
% changing/setting the style of state line 
\newcommand{\ChgStateLineStyle}[1]{\renewcommand{\StateLineSty}{#1}}
\newcommand{\RstStateLineStyle}{\ChgStateLineStyle{\StateLineStyle}}
\newcommand{\SetStateLineStyle}[1]%
   {\renewcommand{\StateLineStyle}{#1}\RstStateLineStyle}
% changing/setting the color of state line
\newcommand{\ChgStateLineColor}[1]{\renewcommand{\StateLineCol}{#1}}
\newcommand{\RstStateLineColor}{\ChgStateLineColor{\StateLineColor}}
\newcommand{\SetStateLineColor}[1]%
   {\renewcommand{\StateLineColor}{#1}\RstStateLineColor}
% changing/setting the doubleline status
\newcommand{\StateLineDouble}%
    {\StateLineDbltrue\renewcommand{\StateLineDbl}{true}}
\newcommand{\StateLineSimple}%
    {\StateLineDblfalse\renewcommand{\StateLineDbl}{false}}
%%%
\newcommand{\FixStateLineDouble}[2]%
   {\renewcommand{\SttLineDblCoef}{#1}%
    \renewcommand{\SttLineDblSep}{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{State drawing style}%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Switching between simple and double line is made by adding style,
% not by setting parameters
\newpsstyle{VCStateStyle}%
        {framesep=0pt,%
         fillstyle=\StateBkgdSty,%
	 fillcolor=\StateBkgdCol,% 
         linewidth=\StateLineWid,%
	 linestyle=\StateLineSty,%
	 linecolor=\StateLineCol,%
         border=\SttBorderWidth,%
         bordercolor=\SttBorderColor,%
	 dimen=\SttDimen,%
         doubleline=false,%\StateLineDbl
         cornersize=\StateCornerRounding,%
	 linearc=\StateCornerRadEff,%
	 framearc=\StateCornerRelRad}
\newpsstyle{VCStateDblStyle}% ATTN New version: incremental style
        {%                   
	 doubleline=true,%\StateLineDbl
         linewidth=\SttLineDblCoef\StateLineWid,%
	 doublesep=\SttLineDblSep\StateLineWid,%
	 doublecolor=\StateBkgdCol,%
	 dimen=\SttDblLineDimen}
\newpsstyle{VCHiddenStateStyle}% ATTN New version: incremental style
        {%                   
         linestyle=none,%
         fillstyle=none}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% new version
\newcommand{\SttStyle}%
   {%
    \ifthenelse{\equal{\VCSttSize}{small}}% 
       {\renewcommand{\StateBkgdSty}{\SmallStateBkgdStyle}%
        \renewcommand{\StateBkgdCol}{\SmallStateBkgdColor}}%
       {}%  
    \psset{style=VCStateStyle}%
    \ifStateLineDbl\psset{style=VCStateDblStyle}\fi%
    \ifVCShowStt\else\psset{style=VCHiddenStateStyle}\fi%
   }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%% TO BE FIXED
%%%   Variable state with double line
%%%   may change the policy of drawing states with double line
%%%   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% VCSG-state-labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state label parameters}%%%%%
% flags
\newif\ifVCRigidStateLabel
\newcommand{\RigidStateLabel}{\VCRigidStateLabeltrue}
\newcommand{\SwivelStateLabel}{\VCRigidStateLabelfalse}
\newif\ifVCStateLabelOnBaseLine
\newcommand{\AlignedStateLabel}{\VCStateLabelOnBaseLinetrue}
\newcommand{\FloatingStateLabel}{\VCStateLabelOnBaseLinefalse}
\newif\ifVCStateLabelInside
\newcommand{\StateLabelInside}{\VCStateLabelInsidetrue}
\newcommand{\StateLabelAside}{\VCStateLabelInsidefalse}
% parameters
\newcommand{\StateLabelColor}{}\newcommand{\StateLabelCol}{}
\newcommand{\StateLabelScale}{}\newcommand{\StateLabelSca}{}
\newcommand{\StateLabelSize}{}\newcommand{\StateLabelSz}{}
\newcommand{\StateLabelStyle}{}\newcommand{\StateLabelSty}{}
% 050302 text mode
\newcommand{\SttLblMode}{} % Internal variable
% parameters for aside labels
\newcommand{\AsideLabelDirct}{}\newcommand{\AsideLabelDir}{}
\newlength{\AsideLabelDistn}{}\newlength{\AsideLabelDst}{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state label changing/setting macros}%%%%%
% changing/setting the label color
\newcommand{\ChgStateLabelColor}[1]{\renewcommand{\StateLabelCol}{#1}}
\newcommand{\RstStateLabelColor}{\ChgStateLabelColor{\StateLabelColor}}
\newcommand{\SetStateLabelColor}[1]%
    {\renewcommand{\StateLabelColor}{#1}\RstStateLabelColor}
% changing/setting the label scale
\newcommand{\ChgStateLabelScale}[1]{\renewcommand{\StateLabelSca}{#1}}
\newcommand{\RstStateLabelScale}{\ChgStateLabelScale{1}}
\newcommand{\SetStateLabelScale}[1]%
   {\renewcommand{\StateLabelScale}{#1}\RstStateLabelScale}
% changing/setting the label size
\newcommand{\ChgStateLabelSize}[1]{\renewcommand{\StateLabelSz}{#1}}
\newcommand{\RstStateLabelSize}{\ChgStateLabelSize{\StateLabelSize}}
\newcommand{\SetStateLabelSize}[1]%
    {\renewcommand{\StateLabelSize}{#1}\RstStateLabelSize}
% changing/setting the label style
\newcommand{\ChgStateLabelStyle}[1]{\renewcommand{\StateLabelSty}{#1}}
\newcommand{\RstStateLabelStyle}{\ChgStateLabelStyle{\StateLabelStyle}}
\newcommand{\SetStateLabelStyle}[1]%
    {\renewcommand{\StateLabelStyle}{#1}\RstStateLabelStyle}
% setting the label text mode %%% processed differently
\newcommand{\StateLabelModeMath}{\renewcommand{\SttLblMode}{$}}%
\newcommand{\StateLabelModeText}{\renewcommand{\SttLblMode}{}}%
% changing/setting the direction of the label aside
\newcommand{\ChgAsideLabelDirct}[1]{\renewcommand{\AsideLabelDir}{#1}}
\newcommand{\RstAsideLabelDirct}{\ChgAsideLabelDirct{\AsideLabelDirct}}
\newcommand{\SetAsideLabelDirct}[1]%
   {\renewcommand{\AsideLabelDirct}{#1}\RstAsideLabelDirct}
% changing/setting the distance of the label aside 
\newcommand{\ChgAsideLabelDistn}[1]%
   {\setlength{\AsideLabelDst}{#1\AsideLabelDistn}}  
\newcommand{\RstAsideLabelDistn}{\ChgAsideLabelDistn{1}}
\newcommand{\SetAsideLabelDistn}[1]% ATTN the parameter is a length
   {\setlength{\AsideLabelDistn}{#1}\RstAsideLabelDistn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{dimmed states}%%%%
%%%  Dimmed states (e.g. for non accessible states)
\newcommand{\DimStateLineStyle}{} 
\newcommand{\DimStateLineCoef}{} 
\newcommand{\DimStateLineColor}{}
\newcommand{\DimStateBkgdColor}{}
\newcommand{\DimStateLabelColor}{}
%%% establishing the dimmed style
\newcommand{\DimState}%
   {\ChgStateLineStyle{\DimStateLineStyle}%
    \ChgStateLineWidth{\DimStateLineCoef}%
    \ChgStateLineColor{\DimStateLineColor}%
    \ChgStateBkgdColor{\DimStateBkgdColor}%
    \ChgStateLabelColor{\DimStateLabelColor}}
%
\newcommand{\SetDimStatePmts}[5]%
   {\renewcommand{\DimStateLineStyle}{#1}%
    \renewcommand{\DimStateLineCoef}{#2}%
    \renewcommand{\DimStateLineColor}{#3}%
    \renewcommand{\DimStateLabelColor}{#4}%
    \renewcommand{\DimStateBkgdColor}{#5}%
    \renewcommand{\DimState}%
       {\ChgStateLineStyle{\DimStateLineStyle}%
        \ChgStateLineWidth{\DimStateLineCoef}%
        \ChgStateLineColor{\DimStateLineColor}%
        \ChgStateBkgdColor{\DimStateBkgdColor}%
        \ChgStateLabelColor{\DimStateLabelColor}}%
    }
%
\newcommand{\UnDimState}%
   {\RstStateLineStyle%
    \RstStateLineWidth%
    \RstStateLineColor%
    \RstStateBkgdColor%
    \RstStateLabelColor}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% restoring state parameters and thus 
%%% initializing the internal parameters to the default values
%%% TO BE FIXED  The initial values of the flags are not stored
%%%              and thus not restored
\newcommand{\RstState}%
  {\RstStateLineWidth%
   \RstStateLineStyle\RstStateLineColor%
   \RstStateBkgdStyle\RstStateBkgdColor%
   \RstStateLabelColor\RstStateLabelScale%
   \RstStateLabelSize\RstStateLabelStyle%
   \RstAsideLabelDirct\RstAsideLabelDistn%
  }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state label parameter computation}%%%%%
% extra space parameters
\newlength{\ExtraSpaceForCrcState}
\newlength{\ExtraSpaceForOvlState}
\newlength{\ExtraSpaceForRctState}
%
\newlength{\LabelBoxWidth}\newlength{\LabelBoxHeight}
\newcommand{\NulLabelBoxWidth}{\setlength{\LabelBoxWidth}{0pt}}
\newcommand{\NulLabelBoxHeight}{\setlength{\LabelBoxHeight}{0pt}}
%%%
% compose the label at the right scale, with the right size
% and in the right style
\newcommand{\SizedStateLabel}[1]%
    {\scalebox{\StateLabelSca}%
       {\scalebox{\StateLabelScale}%
	  {\StateLabelSz \SttLblMode\StateLabelSty{#1}\SttLblMode}}}
%%%
% compute the width of the composed label, 
% adjusted according to the shape of the state
\newcommand{\ComputLabelBoxWnH}[1]%
    {%
     \ifVCStateLabelInside%
        \settowidth{\LabelBoxWidth}{\SizedStateLabel{#1}}% width of lbl                  
        \settodepth{\VCSGTmpLength}{\SizedStateLabel{#1}}	
        \settoheight{\LabelBoxHeight}{\SizedStateLabel{#1}}%                  
        \addtolength{\LabelBoxHeight}{\VCSGTmpLength}%height of label
% add extra space, according to the shape
	\ifthenelse{\equal{\VCSttShp}{circle}}% 
           {\addtolength{\LabelBoxWidth}{\ExtraSpaceForCrcState}%
            \addtolength{\LabelBoxHeight}{\ExtraSpaceForCrcState}}%
            {\ifthenelse{\equal{\VCSttShp}{square}}%\or\equal{\VCSttShp}{rectangle}mystery
               {\addtolength{\LabelBoxWidth}{\ExtraSpaceForRctState}%
                \addtolength{\LabelBoxHeight}{\ExtraSpaceForRctState}}%
                {\ifthenelse{\equal{\VCSttShp}{rectangle}}%
                   {\addtolength{\LabelBoxWidth}{\ExtraSpaceForRctState}%
                    \addtolength{\LabelBoxHeight}{\ExtraSpaceForRctState}}%
                   {\ifthenelse{\equal{\VCSttShp}{oval}}% 
                      {\addtolength{\LabelBoxWidth}{\ExtraSpaceForOvlState}%
                       \addtolength{\LabelBoxHeight}{\ExtraSpaceForOvlState}}%
		      {ErrSttShape}%
                    }%
                 }%
	     }%
     \else% set size to 0
        \NulLabelBoxWidth\NulLabelBoxHeight%
     \fi
     }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compute the shift for labels on baseline 
\newlength{\VertShiftH}\newlength{\VertShiftD}\newlength{\VertShift}%
\newcommand{\VCSFixVertShift}%
   {\settoheight{\VertShiftH}%
      {{\StateLabelSz \SttLblMode\StateLabelSty{\{}\SttLblMode}}%
    \settodepth{\VertShiftD}%
      {{\StateLabelSz \SttLblMode\StateLabelSty{\{}\SttLblMode}}%
    \setlength{\VertShift}{.5\VertShiftD-.5\VertShiftH}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compute the distance for side labels 
\newlength{\AsdLblDst}%
\newcommand{\VCSFixAsdLblDst}%
   {\VCSGGreaterLgt{\LastSttDrawnWidth}{\LastSttDrawnHeight}{\VCSGTmpLength}%
    \CorrPosSttIntDim{\VCSGTmpLength}%
    \setlength{\AsdLblDst}{.5\VCSGTmpLength}%
    \addtolength{\AsdLblDst}{\AsideLabelDst}%
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{state label writing}%%%%%
\newcommand{\WriteStateLabel}[2]%
    {\ifVCShowStt%
        \ifVCStateLabelInside%
           \rput#2{\makebox[0pt]{\WrtStateLabelIns{#1}}}%
        \else%
           \rput#2{\makebox[0pt]{\WrtStateLabelAsd{#1}}}%
        \fi%
     \fi}%
\newcommand{\WrtStateLabelIns}[1]%
    {\ifVCRigidStateLabel%
       \ifVCStateLabelOnBaseLine%
         {\VCSFixVertShift%
	  \textcolor{\StateLabelCol}%
	    {\scalebox{\StateLabelSca}%
               {\scalebox{\StateLabelScale}%
                  {\rput[B]{*0}(0,\VertShift){\WrtSttLbl{#1}}}}}}%
       \else
         {%
          \textcolor{\StateLabelCol}%
	     {\scalebox{\StateLabelSca}%
                {\scalebox{\StateLabelScale}%
                   {\rput{*0}(0,0){\WrtSttLbl{#1}}}}}}%
       \fi
     \else% TO BE FIXED  StateLabelOnBaseLine should be active
       {%
        \textcolor{\StateLabelCol}%
	  {\scalebox{\StateLabelSca}%
             {\scalebox{\StateLabelScale}%
                {\rput{0}(0,0){\WrtSttLbl{#1}}}}}}%
     \fi}
\newcommand{\WrtStateLabelAsd}[1]%
    {\VCSFixAsdLblDst%
     \ifVCRigidStateLabel%
        {\uput{\AsdLblDst}[\AsideLabelDir](0,0)%
           {\textcolor{\StateLabelCol}%
              {\scalebox{\StateLabelSca}%
                 {\scalebox{\StateLabelScale}%
                     {\WrtSttLbl{#1}}}}}}%
     \else% 
        {\uput{\AsdLblDst}[\AsideLabelDir](0,0)%
           {\textcolor{\StateLabelCol}%
              {\scalebox{\StateLabelSca}%
                 {\scalebox{\StateLabelScale}%
                    {\WrtSttLbl{#1}}}}}}%
     \fi}
\newcommand{\WrtSttLbl}[1]%
  {\StateLabelSz\SttLblMode\StateLabelSty{\VCLbl{#1}}\SttLblMode}%
% \newcommand{\VCLbl}[1]%
%    {\ifthenelse{\lengthtest{\LblBxLnWd = 0pt}}%
%       {#1}%
%       {\psframebox%
%           [doubleline=false,%
%            fillstyle=none,%
%            linestyle=solid,%
%            linecolor=\LblBxLnClr,%
%            linewidth=\LblBxLnWd,%
%            linearc=0pt,dimen=outer]%
%           {#1}}%
%     }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
\newcommand{\VCPutStateLabel}[2]{\rput#1{\WrtSttLbl{#2}}}
\newcommand{\AsideStateLabel}[2]%
    {\SpecialCoor%
     \rput(#1){\makebox[0pt]{\WrtStateLabelAsd{#2}}}%
     \NormalCoor%
     }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{construction lines}%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% construction line parameter
\newcommand{\SqrSttCtrClr}{}
\newcommand{\LblBxLnClr}{}
\newcommand{\PhtSttLnClr}{}
\newlength{\SqrSttCtr}
\newlength{\LblBxLnWd}
\newlength{\PhtSttLnWd}
\newlength{\PhtSttCtr}
\newlength{\PhtSttInt}
% construction line commands
\newcommand{\CtrBxLblOn}{\setlength{\LblBxLnWd}{0.3pt}}
\newcommand{\CtrBxLblOff}{\setlength{\LblBxLnWd}{0pt}}
\newcommand{\CtrSqrSttOn}{\setlength{\SqrSttCtr}{0.3pt}}
\newcommand{\CtrSqrSttOff}{\setlength{\SqrSttCtr}{0pt}}
\newcommand{\CtrPhtSttOn}{\setlength{\PhtSttLnWd}{0.3pt}}
\newcommand{\CtrPhtSttOff}{\setlength{\PhtSttLnWd}{0pt}}
% construction line functions
% Draw a box around the parameter (originaly a label, hence the name) 
% when the length \LblBxLnWd has been given a value different from 0 
\newcommand{\VCLbl}[1]%
   {\ifthenelse{\lengthtest{\LblBxLnWd = 0pt}}%
      {#1}%
      {\psframebox%
          [doubleline=false,%
           fillstyle=none,%
           linestyle=solid,%
           linecolor=\LblBxLnClr,%
           linewidth=\LblBxLnWd,%
           linearc=0pt,dimen=outer]%
          {#1}}%
    }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{internal state parameters}%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% internal parameters
\newlength{\SttIntDiamtr}
\newlength{\SttIntWidth}
\newlength{\SttIntHeight}
\newlength{\OvlSttIntWidth}
\newlength{\OvlSttIntHeight}
\newlength{\StateVarWidth}
% twice the distance between the center of state
% and the centers of the phantom states 
\newlength{\SttVarWidthShift}
\newlength{\SttVarHeightShift}
%%%
\newlength{\ActiveLineWidth}
\newcommand{\ActiveDimen}{}
\newcommand{\CorrNegSttIntDim}[1]%
    {\ifStateLineDbl%
        \renewcommand{\ActiveDimen}{\SttDblLineDimen}%
	\setlength{\ActiveLineWidth}{\SttLineDblCoef\StateLineWid}%
	\addtolength{\ActiveLineWidth}{\SttLineDblCoef\StateLineWid}%
	\addtolength{\ActiveLineWidth}{\SttLineDblSep\StateLineWid}%
     \else%
        \renewcommand{\ActiveDimen}{\SttDimen}%
	\setlength{\ActiveLineWidth}{\StateLineWid}%
     \fi%
     \ifthenelse{\equal{\ActiveDimen}{outer}}%
        {\addtolength{#1}{-2\StateLineWid}}%
        {\ifthenelse{\equal{\ActiveDimen}{middle}}%
            {\addtolength{#1}{-\StateLineWid}}%
            {}%
	 }%
    }
\newcommand{\CorrPosSttIntDim}[1]%
    {\ifStateLineDbl%
        \renewcommand{\ActiveDimen}{\SttDblLineDimen}%
        \setlength{\ActiveLineWidth}{\SttLineDblCoef\StateLineWid}%
        \addtolength{\ActiveLineWidth}{\SttLineDblCoef\StateLineWid}%
        \addtolength{\ActiveLineWidth}{\SttLineDblSep\StateLineWid}%
     \else%
        \renewcommand{\ActiveDimen}{\SttDimen}%
        \setlength{\ActiveLineWidth}{\StateLineWid}%
     \fi%
     \ifthenelse{\equal{\ActiveDimen}{outer}}%
        {\addtolength{#1}{2\StateLineWid}}%
        {\ifthenelse{\equal{\ActiveDimen}{middle}}%
            {\addtolength{#1}{\StateLineWid}}%
            {}%
         }%
    }
%%%
\newcommand{\ComputSttIntDimension}%
    {%
     \setlength{\SttIntWidth}{\StateDia}%
     \setlength{\SttIntHeight}{\StateDia}%
     \setlength{\PhtSttInt}{\StateDia}%
     \addtolength{\PhtSttInt}{-2\PhtSttLnWd}
     \ifthenelse{\equal{\VCSttShp}{circle}\or\equal{\VCSttShp}{square}}%
       {}% do nothing
%        {\ifthenelse{\equal{\VCSttShp}{square}}%
%          {}% do nothing
	 {\ifthenelse{\equal{\VCSttShp}{rectangle}}%
	   {\ifthenelse{\VCSGCmdPosTst{\RectangleStateRat}}%
	     {\setlength{\SttIntWidth}{\RectangleStateRat\StateDia}}%
             {\setlength{\SttIntHeight}{\RectangleStateRat\StateDia}%
              \setlength{\SttIntHeight}{-\SttIntHeight}}%
	   }%
	   {\ifthenelse{\equal{\VCSttShp}{oval}}%
	     {\ifthenelse{\VCSGCmdPosTst{\OvalStateRat}}%
	       {\setlength{\SttIntWidth}{\OvalStateRat\StateDia}}%
               {\setlength{\SttIntHeight}{\OvalStateRat\StateDia}%
		\setlength{\SttIntHeight}{-\SttIntHeight}}%
             }%
	     {ErrSttShape}%
           }%
%          }%
       }%
     \CorrNegSttIntDim{\SttIntWidth}%
     \CorrNegSttIntDim{\SttIntHeight}%
    }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{Internal state drawing commands}%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength{\IntCrossTmp}%
\newcommand{\IntCross}[3]%
   {\setlength{\IntCrossTmp}{#1}\addtolength{\IntCrossTmp}{-#3}%
    {\color{\SqrSttCtrClr}%
     {\protect\rule[-.5#3]{.5\IntCrossTmp}{#3}%
     \protect\rule[-.5#2]{#3}{#2}%
     \protect\rule[-.5#3]{.5\IntCrossTmp}{#3}}%
    }}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% defines and draws a circle state
\newcommand{\VCSGCrcState}[3]{\rput#1{\Cnode[radius=.5#3](0,0){#2}}}
% defines and draws a square state
\newcommand{\VCSGSqrState}[4]%
   {\rput#1{\rnode{#2}{\psframebox{\IntCross{#3}{#4}{\SqrSttCtr}}}}}
% defines and draws an oval state
\newcommand{\VCSGOvlState}[4]%
   {\setlength{\OvlSttIntWidth}{\HSQRTwo#3}%
    \setlength{\OvlSttIntHeight}{\HSQRTwo#4}%
    \rput#1{\ovalnode{#2}%
               {\IntCross{\OvlSttIntWidth}{\OvlSttIntHeight}{\SqrSttCtr}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% call for the drawing of a state of normal size
\newcommand{\DrawState}[2]%
   {\SttStyle%
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\VCSGCrcState{#1}{#2}{\StateDia}}%
       {\ifthenelse{\equal{\VCSttShp}{square}\or\equal{\VCSttShp}{rectangle}}%
           {\VCSGSqrState{#1}{#2}{\SttIntWidth}{\SttIntHeight}}%
           {\ifthenelse{\equal{\VCSttShp}{oval}}%
               {\VCSGOvlState{#1}{#2}{\SttIntWidth}{\SttIntHeight}}%
               {ErrorStateShape \VCSttShp}%
            }%
        }%
    }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ProcessState}[3]%
   {%
    \RazSttVar
    \ifVCSizedNode%
 	\ProcessSizedState{#1}{#2}{#3}%   
    \else
 	\ProcessSizelessState{#1}{#2}{#3}%   
    \fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\State}[3][{}]%
   {\renewcommand{\VCSttShp}{\VCSttShape}\ProcessState{#1}{#2}{#3}}  
\newcommand{\CrcState}[3][{}]%
   {\renewcommand{\VCSttShp}{circle}\ProcessState{#1}{#2}{#3}}   
\newcommand{\OvlState}[3][{}]%
   {\renewcommand{\VCSttShp}{oval}\ProcessState{#1}{#2}{#3}}   
\newcommand{\SqrState}[3][{}]%
   {\renewcommand{\VCSttShp}{square}\ProcessState{#1}{#2}{#3}}   
\newcommand{\RctState}[3][{}]%
   {\renewcommand{\VCSttShp}{rectangle}\ProcessState{#1}{#2}{#3}}   
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%\section{variable states}%%
%%%
%  A flag for the variable state plolicy:
%    true:  size of label control whether state is "Var" or not
%    false: state is "Var" only when declared so
\newif\ifAdjstSttFlg 
\newcommand{\SelfAdjustState}{\AdjstSttFlgtrue}
\newcommand{\FixedSizeState}{\AdjstSttFlgfalse}
%  Mode of variable states
\newcommand{\VCSttVarMode}{}
% horizontal, vertical (Two phantom states created) 
% total        (Four phantom states created)
% hypertotal   (Eight phantom states created) -- not implemented
% homothetic   (No phantom states created)
\newcommand{\HorizontalStateVarMode}{\renewcommand{\VCSttVarMode}{horizontal}}
\newcommand{\VerticalStateVarMode}{\renewcommand{\VCSttVarMode}{vertical}}
\newcommand{\TotalStateVarMode}{\renewcommand{\VCSttVarMode}{total}}
\newcommand{\HomotheticStateVarMode}{\renewcommand{\VCSttVarMode}{homothetic}}
%
\newcommand{\StateVarMode}[1]{\renewcommand{\VCSttVarMode}{#1}}
%%%
%  Flags to remember if the last state drawn is a variable state
%  commands are for internal use
\newif\ifVCSttVar  
\newif\ifVCSttVarH  
\newif\ifVCSttVarV  
\newcommand{\RazSttVar}%
   {\VCSttVarfalse\VCSttVarHfalse\VCSttVarVfalse}
\newcommand{\IsSttVar}{\VCSttVartrue}
\newcommand{\IsSttVarH}{\VCSttVarHtrue}
\newcommand{\IsSttVarV}{\VCSttVarVtrue}
\RazSttVar % initialization, as it is internal 
%%%
% In case of Circle State, variable states are made by rectangle,
% with corner rounded with a radius equal to the half of the height.
\newpsstyle{CrcStateVarStyle}%
        {%
         cornersize=absolute,%
	 linearc=0.5\StateDia}%
%%% syle for the phantom states
\newpsstyle{NoPhtStateStyle}%
        {framesep=0pt,%
         fillstyle=none,%
         linewidth=\PhtSttLnWd,%
         linestyle=none,%
         linecolor=green,%
         doubleline=false,%
         dimen=outer}%
\newpsstyle{PhtStateStyle}%
        {framesep=0pt,%
         fillstyle=none,%
         linewidth=\PhtSttLnWd,%
         linestyle=dashed,%
         linecolor=\PhtSttLnClr,%
         doubleline=false,%
         dimen=outer}%
%%%
\newcommand{\CrcSttVarStyle}%
   {\ifVCShowStt\psset{style=CrcStateVarStyle}%
        \else\psset{style=VCSGHiddenStateStyle}\fi}
\newcommand{\PhtSttVarStyle}%
   {\ifVCShowStt%
       \ifthenelse{\lengthtest{\PhtSttLnWd = 0pt}}%
           {\psset{style=NoPhtStateStyle}}%
           {\psset{style=PhtStateStyle}}%
        \else\psset{style=VCSGHiddenStateStyle}\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% call for the drawing of a state of variable size
%%% Choice between the var modes
\newcommand{\DrawStateVar}[2]% 
   {\SttStyle%
    \ifthenelse{\equal{\VCSttVarMode}{horizontal}}%
       {\ifVCSttVarH\DrawStateVarH{#1}{#2}\else\DrawState{#1}{#2}\fi}%
       {\ifthenelse{\equal{\VCSttVarMode}{vertical}}%
           {\ifVCSttVarV\DrawStateVarV{#1}{#2}\else\DrawState{#1}{#2}\fi}%
           {\ifthenelse{\equal{\VCSttVarMode}{total}}%
               {\DrawStateVarT{#1}{#2}}%
               {\ifthenelse{\equal{\VCSttVarMode}{homothetic}}%
                   {\DrawStateVarM{#1}{#2}}%
                   {ErrorStateVarMode \VCSttVarMode}%
               }%
           }%
       }%
   }%
%%% Square phantom state
\newcommand{\SqrPhtStt}{\psframebox{\IntCross{\PhtSttInt}{\PhtSttInt}{\PhtSttCtr}}}
%%% Choice between the shapes
\newcommand{\DrawStateVarH}[2]%
   {\SttStyle%
    \setlength{\SttVarWidthShift}{\LastSttDrawnWidth}%
    \addtolength{\SttVarWidthShift}{-\StateDia}% 
    \CorrPosSttIntDim{\SttVarWidthShift}% 
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\CrcSttVarStyle%
        \VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
        \PhtSttVarStyle%
        \rput#1{\Cnode[radius=.5\StateDia](.5\SttVarWidthShift,0){#2e}}%
        \rput#1{\Cnode[radius=.5\StateDia](-.5\SttVarWidthShift,0){#2w}}%
        }%
       {\ifthenelse{\equal{\VCSttShp}{square}\or\equal{\VCSttShp}{rectangle}}%
           {\VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
            \PhtSttVarStyle%
            \rput#1{\rput(.5\SttVarWidthShift,0){\rnode{#2e}{\SqrPhtStt}}}%
            \rput#1{\rput(-.5\SttVarWidthShift,0){\rnode{#2w}{\SqrPhtStt}}}%
            }%
           {\ifthenelse{\equal{\VCSttShp}{oval}}%
                {\VCSGOvlState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}}%
                {ErrorStateShape \VCSttShp}%
            }%
       }%
   }%
%%% Choice between the shapes
\newcommand{\DrawStateVarV}[2]%
   {\SttStyle%
    \setlength{\SttVarHeightShift}{\LastSttDrawnHeight}%
    \addtolength{\SttVarHeightShift}{-\StateDia}% 
    \CorrPosSttIntDim{\SttVarHeightShift}% 
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\CrcSttVarStyle%
        \VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
        \PhtSttVarStyle%
        \rput#1{\Cnode[radius=.5\StateDia](0,.5\SttVarHeightShift){#2n}}%
        \rput#1{\Cnode[radius=.5\StateDia](0,-.5\SttVarHeightShift){#2s}}%
        }%
       {\ifthenelse{\equal{\VCSttShp}{square}\or\equal{\VCSttShp}{rectangle}}%
           {\VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
            \PhtSttVarStyle%
            \rput#1{\rput(0,.5\SttVarHeightShift){\rnode{#2n}{\SqrPhtStt}}}%
            \rput#1{\rput(0,-.5\SttVarHeightShift){\rnode{#2s}{\SqrPhtStt}}}%
            }%
           {\ifthenelse{\equal{\VCSttShp}{oval}}%
                {\VCSGOvlState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}}%
                {ErrorStateShape \VCSttShp}%
            }%
       }%
   }%
%%% Choice between the shapes
\newcommand{\DrawStateVarT}[2]%
   {\SttStyle%
    \setlength{\SttVarWidthShift}{\LastSttDrawnWidth}%
    \addtolength{\SttVarWidthShift}{-\StateDia}% 
    \CorrPosSttIntDim{\SttVarWidthShift}% 
    \setlength{\SttVarHeightShift}{\LastSttDrawnHeight}%
    \addtolength{\SttVarHeightShift}{-\StateDia}% 
    \CorrPosSttIntDim{\SttVarHeightShift}% 
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\CrcSttVarStyle%
        \VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
        \SttStyle\PhtSttVarStyle%
        \rput#1{\rput(.5\SttVarWidthShift,0){\rnode{#2e}{\SqrPhtStt}}}%
        \rput#1{\rput(-.5\SttVarWidthShift,0){\rnode{#2w}{\SqrPhtStt}}}%
        \rput#1{\rput(0,.5\SttVarHeightShift){\rnode{#2n}{\SqrPhtStt}}}%
        \rput#1{\rput(0,-.5\SttVarHeightShift){\rnode{#2s}{\SqrPhtStt}}}%
        }%
       {\ifthenelse{\equal{\VCSttShp}{square}\or\equal{\VCSttShp}{rectangle}}%
           {\VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}%
            \PhtSttVarStyle%
            \rput#1{\rput(.5\SttVarWidthShift,0){\rnode{#2e}{\SqrPhtStt}}}%
            \rput#1{\rput(-.5\SttVarWidthShift,0){\rnode{#2w}{\SqrPhtStt}}}%
            \rput#1{\rput(0,.5\SttVarHeightShift){\rnode{#2n}{\SqrPhtStt}}}%
            \rput#1{\rput(0,-.5\SttVarHeightShift){\rnode{#2s}{\SqrPhtStt}}}%
            }%
            {\ifthenelse{\equal{\VCSttShp}{oval}}%
                {\VCSGOvlState{#1}{#2}{\LastSttDrawnWidth}{\LastSttDrawnHeight}}%
                {ErrorStateShape \VCSttShp}%
             }%
        }%
    }%
%%% Choice between the shapes
\newcommand{\DrawStateVarM}[2]%
   {\SttStyle%
    \ifthenelse{\equal{\VCSttShp}{circle}}%
       {\VCSGGreaterLgt{\LastSttDrawnWidth}{\LastSttDrawnHeight}{\VCSGTmpLength}%
        \VCSGCrcState{#1}{#2}{\VCSGTmpLength}}%
       {\ifthenelse{\equal{\VCSttShp}{square}}%
           {\VCSGGreaterLgt{\LastSttDrawnWidth}{\LastSttDrawnHeight}{\VCSGTmpLength}%
            \VCSGSqrState{#1}{#2}{\VCSGTmpLength}{\VCSGTmpLength}}%%
           {\ifthenelse{\equal{\VCSttShp}{rectangle}}%
               {\ifthenelse{\VCSGCmdPosTst{\RectangleStateRat}}%
                   {\setlength{\VCSGTmpLength}{\RectangleStateRat\LastSttDrawnHeight}%
                    \ifthenelse{\lengthtest{\VCSGTmpLength>\LastSttDrawnWidth}%
                                \or\lengthtest{\VCSGTmpLength=\LastSttDrawnWidth}}%
                        {\VCSGSqrState{#1}{#2}{\VCSGTmpLength}{\LastSttDrawnHeight}}%
                        {\setlength{\VCSGTmpLength}{\LastSttDrawnWidth*\ratio{1pt}{\RectangleStateRat pt}}%
                         \VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\VCSGTmpLength}}%%
                    }%    
                   {\setlength{\VCSGTmpLength}{-\RectangleStateRat\LastSttDrawnWidth}%
                    \ifthenelse{\lengthtest{\VCSGTmpLength>\LastSttDrawnHeight}%
                                \or\lengthtest{\VCSGTmpLength=\LastSttDrawnHeight}}%
                        {\VCSGSqrState{#1}{#2}{\LastSttDrawnWidth}{\VCSGTmpLength}}%%
                        {\setlength{\VCSGTmpLength}{\LastSttDrawnHeight*\ratio{1pt}{-\RectangleStateRat pt}}%
                         \VCSGSqrState{#1}{#2}{\VCSGTmpLength}{\LastSttDrawnHeight}}%%
                    }%
                }%
               {\ifthenelse{\equal{\VCSttShp}{oval}}%
                   {\ifthenelse{\VCSGCmdPosTst{\OvalStateRat}}%
                       {\setlength{\VCSGTmpLength}{\OvalStateRat\LastSttDrawnHeight}%
                        \ifthenelse{\lengthtest{\VCSGTmpLength>\LastSttDrawnWidth}%
                                    \or\lengthtest{\VCSGTmpLength=\LastSttDrawnWidth}}%
                           {\setlength{\OvlSttIntWidth}{\HSQRTwo\VCSGTmpLength}%
                            \setlength{\OvlSttIntHeight}{\HSQRTwo\LastSttDrawnHeight}}%
                           {\setlength{\VCSGTmpLength}{\LastSttDrawnWidth*\ratio{1pt}{\OvalStateRat pt}}%
                            \setlength{\OvlSttIntWidth}{\HSQRTwo\LastSttDrawnWidth}%
                            \setlength{\OvlSttIntHeight}{\HSQRTwo\VCSGTmpLength}}}%    
                       {\setlength{\VCSGTmpLength}{-\OvalStateRat\LastSttDrawnWidth}%
                        \ifthenelse{\lengthtest{\VCSGTmpLength>\LastSttDrawnHeight}%
                                    \or\lengthtest{\VCSGTmpLength=\LastSttDrawnHeight}}%
                           {\setlength{\OvlSttIntWidth}{\HSQRTwo\LastSttDrawnWidth}%
                            \setlength{\OvlSttIntHeight}{\HSQRTwo\VCSGTmpLength}}%
                           {\setlength{\VCSGTmpLength}{\LastSttDrawnHeight*\ratio{1pt}{-\OvalStateRat pt}}%
                            \setlength{\OvlSttIntWidth}{\HSQRTwo\VCSGTmpLength}%
                            \setlength{\OvlSttIntHeight}{\HSQRTwo\LastSttDrawnHeight}}}%
                    \rput#1{\ovalnode{#2}{\IntCross{\OvlSttIntWidth}{\OvlSttIntHeight}{\SqrSttCtr}}}%
                    }%
                   {ErrorStateShape \VCSttShp}%
                }%
            }%
        }%
    }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% record the width, and the height, of the composed label
% and whether it makes the state a "variable" one.
\newlength{\LastSttDrawnHeight}
\newlength{\LastSttDrawnWidth}
\newcommand{\FixVarSttDrawingPar}%
    {%
     \RazSttVar%
     \ifthenelse{\lengthtest{\LabelBoxWidth > \SttIntWidth}%
                 \and\(\not\equal{\VCSttVarMode}{vertical}\)}%
        {\IsSttVarH\IsSttVar%
         \setlength{\LastSttDrawnWidth}{\LabelBoxWidth}}%
        {\setlength{\LastSttDrawnWidth}{\SttIntWidth}}%
     \ifthenelse{\lengthtest{\LabelBoxHeight > \SttIntHeight}%
                 \and\(\not\equal{\VCSttVarMode}{horizontal}\)}%
        {\IsSttVarV\IsSttVar%
         \setlength{\LastSttDrawnHeight}{\LabelBoxHeight}}%
        {\setlength{\LastSttDrawnHeight}{\SttIntHeight}}%
    }%
%%%%%\section{process states}%%%%%%%%%%%%%%%%%%%
% the top calling procedure for drawing states
% when entering that procedure, 
% \VCSttShp should be given the right value
\newcommand{\ProcessSizedState}[3]%
    {\ComputSttIntDimension%
     \ComputLabelBoxWnH{#1}%
     \ifAdjstSttFlg 
     \else 
        \NulLabelBoxWidth\NulLabelBoxHeight%
     \fi% 
     \FixVarSttDrawingPar%
     \ifVCSttVar
        \DrawStateVar{#2}{#3}%
     \else
        \DrawState{#2}{#3}%
     \fi%
     \WriteStateLabel{#1}{#2}%
    }%
%%% the same, without the test on AdjstSttFlg
\newcommand{\ProcessSizedStateVar}[3]%
    {\ComputSttIntDimension%
     \ComputLabelBoxWnH{#1}%
     \FixVarSttDrawingPar%
      \ifVCSttVar
         \DrawStateVar{#2}{#3}%
      \else
         \DrawState{#2}{#3}%
      \fi%
     \WriteStateLabel{#1}{#2}%
    }
%%%
\newcommand{\StateVar}[3][{}]%
   {\renewcommand{\VCSttShp}{\VCSttShape}
    \RazSttVar%
    \ifVCSizedNode%
 	\ProcessSizedStateVar{#1}{#2}{#3}%   
    \else
 	\ProcessSizelessState{#1}{#2}{#3}%   
    \fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\FinalSttStyle}%
   {\ifVCShowStt\psset{style=VcsnStateDblStyle}%
    \else\psset{style=VcsnHiddenStateStyle}\fi}
\newcommand{\DotSttStyle}%
   {\ifVCShowStt\psset{style=VcsnVertexStyle}%
        \else\psset{style=VcsnHiddenStateStyle}\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\StateDimen}{}
\newcommand{\StateDblDimen}{}
%
\newcommand{\SetStateFillColor}[1]{\SetStateBkgdColor{#1}}%
\newcommand{\SetStateFillStatus}[1]{\SetStateBkgdStyle{#1}}%
\newcommand{\SmallStateFillColor}{}% apparently not used in 0.4 either
%% state size
\newcommand{\MediumState}{\MediumStates}
\newcommand{\SmallState}{\SmallStates}
\newcommand{\LargeState}{\LargeStates}
%%% hiding--showing
\newcommand{\HideState}{\HideStates}
\newcommand{\ShowState}{\ShowStates}
%%% hiding--showing
\newcommand{\AlignedLabel}{\AlignedStateLabel}
\newcommand{\FloatingLabel}{\FloatingStateLabel}
%%% dim states 
%%% (tricky compatibility: order of parameters has changed!)
\newcommand{\FixDimState}[5]{\SetDimStatePmts{#1}{#3}{#2}{#4}{#5}} 
%%% ecological commands (obsolete from v. 1.0 on -- idem state) 
\newcommand{\StateIF}[3][{}]{\State[#1]{#2}{#3}}%
\newcommand{\StateIFX}[3][{}]{\State[#1]{#2}{#3}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Very Small State   
\newcommand{\VSStateLineCoef}{.6} % coef. for very small state
\newcommand{\VSState}[2]%
    {\renewcommand{\ArrowOnStateCoef}{\ArrowOnVerySmallState}%
     \FixStateDiameter{\VerySmallStateDiameter}%
     \ChgStateLineWidth{\VSStateLineCoef}%
         \State{#1}{#2}%
         \RstStateLineWidth\RstSttDiameter}% mod 020201
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\RigidLabel}{\VCRigidStateLabeltrue}
\newcommand{\SwivelLabel}{\VCRigidStateLabelfalse}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % changing/setting the width of state border 
% %        (the space between state line and the transitions) NON!
% \newcommand{\ChgStateBorderWidth}[1]%
%    {\setlength{\StateBorderWid}{#1\StateBorderWidth}}  
% \newcommand{\RstStateBorderWidth}{\ChgStateBorderWidth{1}}
% \newcommand{\SetStateBorderWidth}[1]% ATTN the parameter is a length
%    {\setlength{\StateBorderWidth}{#1}\RstStateBorderWidth}


==> VCSGPref-beamer.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Package `VauCanSon-G'  version 0.4
%%
%% This is file `VCPref-slides'.
%%
%% IMPORTANT NOTICE:
%%
%% Copyright (C) 2002-2008 Sylvain Lombardy and Jacques Sakarovitch
%%
%% This package may be distributed under the terms of the LaTeX Project
%% Public License, as described in lppl.txt in the base LaTeX distribution.
%% Either version 1.0 or, at your option, any later version.
%%
%% DESCRIPTION:
%%
%%   `VCPref-beamer' contains initial values of VauCanSon-G 
%%   parameters suitable for drawing automata in slides.
%%   Works with package `beamer'; 
%%   smaller scale values than those given in `VCPref-slides'
%%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scales  --- slides settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\LargeScale}{0.85}       
\renewcommand{\MediumScale}{0.6}       
\renewcommand{\SmallScale}{0.4}		
\renewcommand{\TinyScale}{0.30}		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% State aspect
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetStateLineWidth{2pt}
\SetStateLineColor{blue}
\SetStateBkgdColor{Cyan}
\SetStateLabelColor{Sepia}
%%% Dimmed states
\SetDimStatePmts{solid}{1}{YellowOrange}{YellowOrange}{white}
%%%%%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetEdgeLineColor{Mahogany}
\SetEdgeLineWidth{1.2pt}
\SetEdgeLabelColor{OliveGreen}
%%% Dimmed edges
\SetDimEdgePmts{dashed}{1.2}{Apricot}{Apricot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\HideFrame
\HideGrid
\HideName
\MediumState
\MediumPicture
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput


==> VCSGPref-mystyle.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Package VauCanSon-G  version 1.0
%%
%% FILE:    VCPref-mystyle
%%
%% DESCRIPTION:  personal setting of VauCanSon-G's parameters
%%
%  By definiton, an empty file to be customised.
%  
%  VCSG-Preferences.tex is copied after the \endinput
%  andcan be used as a template to write 
%  a customized style of Vaucanson.
%  
%%  
%% DATE:    2012/07/05
%%
%% Copyright (C) 2009-2012 Sylvain Lombardy and Jacques Sakarovitch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-environment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{Scaling matters}%%%%%  
% Inner parameters
\renewcommand{\LargeScale}{0.85}    %float : argument of a \scalebox
\renewcommand{\LargeScaleI}{1.18}
\renewcommand{\MediumScale}{0.6}    %float
\renewcommand{\MediumScaleI}{1.67}
\renewcommand{\SmallScale}{0.5}     %float
\renewcommand{\SmallScaleI}{2}
\renewcommand{\TinyScale}{0.42}     %float
\renewcommand{\TinyScaleI}{2.38}
%
\MediumPictures
\FixVCGridScale{1}
%%%%%\section{Picture directory}%%%%%
% \SetVCDirectory{}  % for record : the definition of \VCDirectory is 
%                    % an initialisation 
%%%%%\section{Picture framing}%%%%%
% Inner parameters
\setlength{\VCFrameLineWidth}{0.6pt}
\renewcommand{\VCFrameLineColor}{black}
\setlength{\VCGridLineWidth}{0.6pt}
\renewcommand{\VCGridLineColor}{black}
%
\SetVCBkgdStyle{solid} % Also set StateBkgd, SmallStateBkgd,
                       % SttBorderColor,EdgeLineBorderColor
\SetVCBkgdColor{white} % and DblEdgeLineColor
%
\HideFrame\HideGrid\HideName
%%%%%\section{Picture drawing call}%%%%%
\FixVerticalPlacement{0.5} %float 
%%%%%\section{VauCanSon-G modes}%%%%%
\Automata 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-states}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%\section{node mode}%%%%%%
% \SizedNodes % for record; not necessary after the call to \Automata 
%%%%%\section{state size}%%%%%%
\setlength{\SmallStateDiameter}{.6cm}
\setlength{\MediumStateDiameter}{1cm}
\setlength{\LargeStateDiameter}{1.2cm}
% \FixStateSizes{.6cm}{.9cm}{1.2cm}{.3cm} would have the same effect
%
% \MediumStates postponed after the definition of loop geometry 
% parameters
%%%%%\section{state shape}%%%%%
\CircleStates
\SetOvalStateRatio{\GoldMeanI}
\SetRectangleStateRatio{\GoldMeanI}
%
\SharpStateCorners 
\StateCornerRoundingAbsolute
\SetStateCornerRelRadius{0}
\SetStateCornerRadius{0.2cm}
%%%%%\section{Hiding -- showing}%%%%%
\ShowStates
%%%%%\section{state background parameters}%%%%%
% for record: setting done when setting the Bkgd of the picture 
% \SetStateBkgdStyle{\VCBkgdStyle}\SetStateBkgdColor{\VCBkgdColor}
% \SetSmallStateBkgdStyle{\VCBkgdStyle}
% \SetSmallStateBkgdColor{\VCBkgdColor}
%%%%%\section{construction line parameters}%%%%%%
\renewcommand{\SqrSttCtrClr}{blue}
\renewcommand{\LblBxLnClr}{red}
\renewcommand{\PhtSttLnClr}{green}
\CtrBxLblOff
\CtrSqrSttOff
\CtrPhtSttOff
\setlength{\PhtSttCtr}{0pt} %%% 
%%%%%\section{state line parameters}%%%%%%
% Inner parameters
\renewcommand{\SttDimen}{outer}
\renewcommand{\SttDblLineDimen}{middle}
\setlength{\SttBorderWidth}{0pt}
% \renewcommand{\SttBorderColor}{\StateBkgdColor} for record
\FixStateLineDouble{0.6}{0.4}  
%%%%%\section{state line parameters}%%%%%%
\SetStateLineWidth{1.8pt}
\SetStateLineStyle{solid}
\SetStateLineColor{black}
%
\StateLineSimple
%%%%%\section{state label parameters}%%%%%
\RigidStateLabel\FloatingStateLabel\StateLabelInside
\SetStateLabelColor{black}
% \SetStateLabelScale{1.667} (set by the scale picture commands)
\SetStateLabelSize{\normalsize}
\StateLabelModeMath
\SetStateLabelStyle{}
\SetAsideLabelDirct{72}
\SetAsideLabelDistn{6pt}
%%% Variable States
% extra space between the label and the state line (to be fixed)
\setlength{\ExtraSpaceForCrcState}{4mm}
\setlength{\ExtraSpaceForOvlState}{2mm}
\setlength{\ExtraSpaceForRctState}{2mm}
% mode initialisation
\HorizontalStateVarMode\SelfAdjustState
%%% Sizeless States
\setlength{\VerySmallStateDiameter}{.3cm}
%%% Dimmed states
% \renewcommand{\DimStateLineStyle}{solid} 
% \renewcommand{\DimStateLineCoef}{1} % 
% \renewcommand{\DimStateLineColor}{gray}
% \renewcommand{\DimStateLabelColor}{gray}
% \renewcommand{\DimStateBkgdColor}{white}
\SetDimStatePmts{solid}{1}{gray}{gray}{white}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   \part{VCSG-edges}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge label drawing macros
\renewcommand{\InOutLbl}[2]{#1\!\mid\! #2} % other ex: {(#1, #2)} 
\renewcommand{\IOL}[2]{#1\!\mid\! #2} % downward compatibility 
\renewcommand{\LblCnnct}{+}
%%% Edge drawing parameters
%%% Line
\SetEdgeLineWidth{1pt}			%% width (length param.)
\SetEdgeLineStyle{solid}		%% aspect
\SetEdgeLineColor{black}		%% color
\EdgeLineSimple
% double line the two coefficients have already been initialised in 
% VCSG-edges.tex in order to avoid deadlock; the call to 
% \FixEdgeLineDouble completes the initialisation
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
\SetDblEdgeLineColor{\VCBkgdColor} %% useless since it has 
              %% already been initialised with the picture background
% border
\EdgeLineBorderOff
\FixEdgeLineBorder{2}{\VCBkgdColor}		%% int,color : coef*\EdgeLineWidth -> width of border
%%% Edge arrow
\ArrowEdge				%% fix the style of arrows
% arrows on simple line 
\SetEdgeArrowWidthBase{2.5pt}
\SetEdgeArrowWidthCoef{2}
\SetEdgeArrowLengthCoef{1.4}
\SetEdgeArrowInsetCoef{0.1}
% idem  \SetEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
% arrows on double line 
\SetDblEdgeArrowWidthBase{2.5pt}
\SetDblEdgeArrowWidthCoef{1.6}
\SetDblEdgeArrowLengthCoef{1.3}
\SetDblEdgeArrowInsetCoef{0.1}
% idem  \SetDblEdgeArrowDimensions{2pt}{3}{1.4}{0.1}  
%%% Edge geometry parameters
\SetEdgeOffset{3pt}
\SetEdgeOffsetCoef{3}
\EdgeOffsetOff
\EdgeOffsetAbs
\SetForthBackEdgeOffsetCoef{2}% coef
\ForthBackOffsetOff
%
\NodeSeparationOff
\SetNodeSep{3pt}
%%% Edge label parameters
\EdgeLabelModeMath
\SetEdgeLabelSize{\normalsize}
\SetEdgeLabelStyle{}
\SetEdgeLabelColor{black}
\SetEdgeLabelScale{1.667}
%%% Edge label boxing parameters
\BoxedEdgeLabelOff
\renewcommand{\BxdEdgLblSep}{5}
\renewcommand{\BxdEdgLblBkg}{white}
\renewcommand{\BxdEdgLblWdt}{1}
\renewcommand{\BxdEdgLblStl}{solid}
\renewcommand{\BxdEdgLblCol}{black}
\renewcommand{\BxdEdgLblDbl}{false}
\renewcommand{\BxdEdgLblRnd}{0}
%%% Edge label geometry parameters
\DirectTransitions
\SetEdgLblPosit{.45}{.55}
\SetArcLblPosit{.4}{.6}
\SetLArcLblPosit{.4}{.6}
\SetLoopLblPosit{.25}{.75}
\SetCLoopLblPosit{.25}{.75}
%
\SetTransLabelSep{8pt}
%
\SwivelEdgeLabel
%%% Dimmed edges
% \renewcommand{\DimEdgeLineStyle}{solid} 
% \renewcommand{\DimEdgeLineCoef}{1.2} 
% \renewcommand{\DimEdgeLineColor}{gray}
% \renewcommand{\DimEdgeLabelColor}{gray}
\SetDimEdgePmts{solid}{1.2}{gray}{gray}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  Initial-final arrow drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\ArrowOnSmallState}{1.2} 		%float
\renewcommand{\ArrowOnMediumState}{1}		%float : coef *\StateDiameter for size of initial and final arrows
\renewcommand{\ArrowOnLargeState}{.8}		%float
% implicit parameter
\renewcommand{\InitialDir}{w}
\renewcommand{\FinalDir}{e}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arc geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetArcAngle{15}
\SetLArcAngle{30}
% Curvature
\SetArcCurvature{0.8}
\SetLArcCurvature{0.8}
% Offset
\SetArcOffset{1pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Loop geometry
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Angle
\SetLoopAngle{30}
\SetCLoopAngle{22}
% Preset sizes
\renewcommand{\LoopOnSmallState}{9.6} 		%float
\renewcommand{\LoopOnMediumState}{7}		%float : curvature
\renewcommand{\LoopOnLargeState}{5.8} 		%float
\renewcommand{\CLoopOnSmallState}{12}		%float
\renewcommand{\CLoopOnMediumState}{8}		%float
\renewcommand{\CLoopOnLargeState}{6}		%float
% Offset
\SetLoopOffset{0pt}
%
\MediumStates
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{backward compatibility}%%%%%%
%%%%%  Obsolete commands from version 0.3, 0.4 and 1.0
%%%%%  kept for backward compatibility
%%%%%  cf users manual for description of compatibilty problems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\StateDimen}{outer}
\renewcommand{\StateDblDimen}{middle}
%
\renewcommand{\EdgeLabelPosit}{.45}   
\renewcommand{\EdgeLabelRevPosit}{.55}
\renewcommand{\ArcLabelPosit}{.40}
\renewcommand{\ArcLabelRevPosit}{.60}
\renewcommand{\LArcLabelPosit}{.40}
\renewcommand{\LArcLabelRevPosit}{.60}
\renewcommand{\LoopLabelPosit}{.25}
\renewcommand{\LoopLabelRevPosit}{.75}
\renewcommand{\CLoopLabelPosit}{.25}
\renewcommand{\CLoopLabelRevPosit}{.75}
%
\renewcommand{\LoopVarAngle}{28}
\renewcommand{\LoopOnVariableState}{5.1} 		%float
\renewcommand{\CLoopOnVariableState}{5.2}		%float
\setlength{\LoopVarOffset}{.7pt}
\renewcommand{\LoopOnVerySmallState}{15} 
% label position on initial-final arrow
\renewcommand{\InitStateLabelPosit}{.1}
\renewcommand{\InitStateLabelRevPosit}{.9}
\renewcommand{\FinalStateLabelPosit}{.9}
\renewcommand{\FinalStateLabelRevPosit}{.1}
%
\renewcommand{\ArrowOnVerySmallState}{5} 	%float
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \MediumStates
%%% Shape
%
%%% Variable States
\HorizontalStateVar\SelfAdjustState
%%% Showing -- hiding states
\ShowState
%%% Line
\renewcommand{\VSStateLineCoef}{.6} % coef. for very small state
%%% Background
%%% Label
%%% Label
\setlength{\VertexLineWidth}{0.6pt}             %% length
\renewcommand{\VertexLineColor}{black}        %% color
\renewcommand{\VertexBkgdStyle}{solid} 
\renewcommand{\VertexBkgdColor}{white}        %% color
\SetStateLabelColor{black}		
\renewcommand{\StateLabelScale}{1.7}
\renewcommand{\StateLabelSca}{1}% processing different from other parameters
\RigidLabel\FloatingLabel
%%% Initialisation
\RstState\RstVertex 
%%%%%%%%%%%%%%
%%%%%\section{edge parameters}%%%%%%%%%%
% Edge aspect
%%%%%%%%%%%%%%
\SetArcAngle{15}			%% int (degree)
\SetLArcAngle{30}			%% int (degree)
\SetArcCurvature{0.8}			%% float
\SetEdgeOffset{0pt}                     %% length
\SetArcOffset{1pt}			%% length
\SetLoopOffset{0pt}			%% length
\renewcommand{\ForthBackEdgeOffset}{5}	%% float : coef*\EdgeLineWidth -> offset
\FixEdgeBorder{2}{white}		%% int,color : coef*\EdgeLineWidth -> width of border
\FixEdgeLineDouble{0.5}{0.6}		%% float : coefs*\EdgeLineWidth -> (width of lines, distance)
%%%%%%%%%%%%%%
% ZZ aspect
%%%%%%%%%%%%%%
\setlength{\ZZSize}{.9cm}		% length : apparent diameter
\renewcommand{\ZZShape}{0.5}		% coef: opening of the ZZ
\SetZZLineWidth{1.7}			% float
\renewcommand{\TransLabelZZCoef}{0.6}	% float : coef*\ZZSize -> distance added for labels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Edge parameters  --- Default settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\InitStateLabelPosit}{.10}
\renewcommand{\InitStateLabelRevPosit}{.90}
\renewcommand{\FinalStateLabelPosit}{.90}
\renewcommand{\FinalStateLabelRevPosit}{.10}
% \SetEdgeArrowWidth{5pt}		%length of the edge arrow
% \SetEdgeArrowLengthCoef{1.4}		%float : coef*\EdgeArrowSizeDim width of EA
% \setlength{\EdgeDblArrowWidth}{5.5pt}		%length : size of EA for double transitions
% \renewcommand{\EdgeDblArrowLengthCoef}{1.7}	%int 
% \SetEdgeArrowInsetCoef{0.1}			%float : coef*\EdgeArrowSizeDim
% \SetEdgeArrowStyle{->}				%style (other styles : <-, |-|, -|,...)
% \renewcommand{\EdgeRevArrowStyle}{<-}           %style for reverse transitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initialization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\SetVCDirectory{}        %default dir=current dir
\HideFrame
\HideGrid
\MediumPicture
\HideName
\RigidLabel
\FullState				%% PlainState
\MediumStates


==> aut_02459mod18_3.tex <==
% \SmallPicture\VCDraw{%
\begin{VCPicture}{(-10,-9)(10,1)}
\FixDimEdge{solid}{1.2}{lightgray}{gray}
% states
\VCPut{(0,0)}{ %tree part
  \State[\epsilon]{(0,0)}{e}
  \State[0]{(-5,-3)}{e0}
  \State[1]{(0,-3)}{e1}
  \State[2]{(5,-3)}{e2}
}
\FixStateDiameter{1.5cm} \ChgStateLabelScale{1.2}

\VCPut{(-9,-8)}{ %end
  \StateVar[\mathcal{P}^{\{0,1\}}_{2}]{(0,0)}{e00}
  \State[\mathcal{P}^{\emptyset}_{2}]{(2,0)}{e01}
  \State[\mathcal{P}^{\emptyset}_{2}]{(4,0)}{e02}
  \State[\mathcal{P}^{\emptyset}_{2}]{(7,0)}{e10}
  \StateVar[\mathcal{P}^{\{0\}}_{2}]{(9,0)}{e11}
  \State[\mathcal{P}^{\emptyset}_{2}]{(11,0)}{e12}
  \StateVar[\mathcal{P}^{\{0\}}_{2}]{(14,0)}{e20}
  \StateVar[\mathcal{P}^{\{1\}}_{2}]{(16,0)}{e21}
  \State[\mathcal{P}^{\emptyset}_{2}]{(18,0)}{e22}
}


% initial--final
\Initial{e} %\Final{C}
\Final{e0}
\Final{e2}
% transitions
%\FixDimEdge{solid}{1}{black}{black}
%\ChgEdgeLineWidth
%\ChgEdgeArrowWidth{7pt}
\EdgeR{e}{e0}{0} \EdgeR{e}{e1}{1} \EdgeL{e}{e2}{2}
\EdgeR{e0}{e00}{0} \EdgeR{e0}{e01}{1} \EdgeL{e0}{e02}{2}
\EdgeR{e1}{e10}{0} \EdgeR{e1}{e11}{1} \EdgeL{e1}{e12}{2}
\EdgeR{e2}{e20}{0} \EdgeR{e2}{e21}{1} \EdgeL{e2}{e22}{2}
%\LoopN{A}{a} \LoopS{C}{d}
%
\end{VCPicture}
% }
% \nopagebreak
% \renewcommand{\frcurrentcaption}{Automate reconnaissant $n\equiv0,2,4,5,9~[18]$}
% \renewcommand{\encurrentcaption}{Automaton accepting $n\equiv0,2,4,5,9~[18]$}


==> aut_1mod4_2.tex <==
% \SmallPicture\VCDraw{
\begin{VCPicture}{(-7,-5)(7,1)}
  \NodeSeparationOff
% states
  \State[A]{(0,0)}{e}

  \State[B]{(-4,-2)}{e0}
  \State[C]{(4,-2)}{e1}

  \State[D]{(-6,-4)}{e00}
  \State[E]{(-2,-4)}{e01}
  \State[F]{(2,-4)}{e10}
  \State[G]{(6,-4)}{e11}

%initial final
  \Initial[n]{e}
  \Final[e]{e10}
  \Final[e]{e1}
%edges
  \FixDimEdge{solid}{1}{black}{black}
  \ChgEdgeLineWidth{3}
  \ChgEdgeArrowWidth{7pt}

  \EdgeR{ee}{e1w}{}
  \EdgeR{e1e}{e11w}{}
  \EdgeR{e0e}{e01w}{}
  \CLoopSE{e11e}{}
  \CLoopSE{e10e}{}  
  \CLoopSE{e00e}{} 
  \CLoopSE{e01e}{}
  \DimEdge
  \EdgeR{ew}{e0e}{}
  \EdgeR{e0w}{e00e}{}
  \EdgeR{e1w}{e10e}{}
  \CLoopSW{e11w}{}
  \CLoopSW{e10w}{}  
  \CLoopSW{e00w}{} 
  \CLoopSW{e01w}{}
\end{VCPicture}
% }
% \renewcommand{\frcurrentcaption}{Automate reconnaissant les entiers congrus à 1 modulo 4 en base 2}
% \renewcommand{\encurrentcaption}{Automaton accepting integers congruent to 1 modulo 4 in base 2}


==> aut_2mod3_2.tex <==

% \SmallPicture\VCDraw{%
\begin{VCPicture}{(-1,-1)(9,4)}
% states

\StateVar[0,0]{(0,0)}{s00}
\StateVar[0,1]{(0,3)}{s01}
\StateVar[1,0]{(4,0)}{s10}
\StateVar[1,1]{(4,3)}{s11}
\StateVar[2,0]{(8,0)}{s20}
\StateVar[2,1]{(8,3)}{s21}

% initial--final
\Initial{s00} %\Final{C}
\Final{s20}\Final{s21}
% transitions
\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3.5}
\ChgEdgeArrowWidth{7pt}

\VArcR[.5]{arcangle=32,ncurv=1.3}{s20}{s01}{}
\VArcR[.5]{arcangle=32,ncurv=1.3}{s01}{s20}{}
%\ArcR{20}{01}{} \ArcR{01}{20}{}
\EdgeBorder
\ArcR{s00}{s11}{} \ArcR{s11}{s00}{}
\ArcR{s10}{s21}{} \ArcR{s21}{s10}{}
\EdgeBorderOff
\DimEdge
\ArcR{s00}{s01}{} \ArcR{s01}{s00}{}
\ArcR{s10}{s11}{} \ArcR{s11}{s10}{}
\ArcR{s20}{s21}{} \ArcR{s21}{s20}{}

%\LoopN{A}{a} \LoopS{C}{d}
%
\end{VCPicture}
% }
%
% \renewcommand\frcurrentcaption{$\mathcal A^2_{3}$}
% \renewcommand\encurrentcaption{$\mathcal A^2_{3}$}

==> aut_2mod3_2_v.tex <==
% \begin{center}
%\centering
% \SmallPicture\VCDraw{%
\begin{VCPicture}{(-1,-1)(9,4)}
% states

\StateVar[0,0]{(0,0)}{s00}
\StateVar[0,1]{(0,3)}{s01}
\StateVar[1,0]{(4,0)}{s10}
\StateVar[1,1]{(4,3)}{s11}
\StateVar[2,0]{(8,0)}{s20}
\StateVar[2,1]{(8,3)}{s21}

% initial--final
\Initial{s00} %\Final{C}
\Final{s20}\Final{s21}
% transitions
\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3}
\EdgeLineDouble
%\ChgEdgeLineStyle{double}
\ChgEdgeArrowWidth{9pt}

%\VArcR[.5]{arcangle=32,ncurv=1.3}{20}{01}{}
%\VArcR[.5]{arcangle=32,ncurv=1.3}{01}{20}{}
%\ArcR{20}{01}{} \ArcR{01}{20}{}

\ArcL{s00}{s10}{} \ArcL{s10}{s20}{} \ArcL{s20}{s00}{}
\ArcL{s11}{s01}{} \ArcL{s21}{s11}{} \ArcL{s01}{s21}{}

\RstEdgeArrowWidth
\EdgeLineSimple
\DimEdge
\ArcR{s00}{s01}{} \ArcR{s01}{s00}{}
\ArcR{s10}{s11}{} \ArcR{s11}{s10}{}
\ArcR{s20}{s21}{} \ArcR{s21}{s20}{}

%\LoopN{A}{a} \LoopS{C}{d}
%
\end{VCPicture}
% }
% % \captionof{figure}{ $\mathcal A^2_{3}$ modifié}
% % \end{center}
% \renewcommand\frcurrentcaption{$\mathcal A^2_{3}$ modifié}
% \renewcommand\encurrentcaption{ modified $\mathcal A^2_{3}$}


==> aut_2mod3_2m.tex <==

% \SmallPicture\VCDraw{
\begin{VCPicture}{(-1,-1)(7,1)}

% states

\State[0]{(0,0)}{s0}
\State[1]{(3,0)}{s1}
\State[2]{(6,0)}{s2}


% initial--final
\Initial{s0} 
\Final{s2}
% transitions
\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3}
\ChgEdgeArrowWidth{7pt}


%\ArcR{20}{01}{} \ArcR{01}{20}{}

\ArcR{s1}{s2}{} \ArcR{s2}{s1}{}
\CLoopS{s0}{}
\DimEdge
\ArcR{s0}{s1}{} \ArcR{s1}{s0}{}
\CLoopS{s2}{}

%\LoopN{A}{a} \LoopS{C}{d}
%
\end{VCPicture}
% }
% \renewcommand{\frcurrentcaption}{ $\mathcal A^{2}_{3}$ minimisé}
% \renewcommand{\encurrentcaption}{ $\mathcal A^{2}_{3}$ minimized}


==> aut_5mod12_2.tex <==
% \SmallPicture\VCDraw{
\begin{VCPicture}{(-6,-5)(14,2)}
\StateVar[A|0]{(4,0.5)}{a}
\StateVar[B|1]{(-3.3,-1.75)}{b}
\StateVar[C|0]{(11,-1.75)}{c}



\VCPut{(-8.8,-4)} {
  \StateVar[D|0]{(0,0)}{d0}
  \StateVar[D|1]{(2.25,0)}{d1}
  \StateVar[D|2]{(4.5,0)}{d2}
}

\VCPut{(-2,-4)} {
  \StateVar[E|0]{(0,0)}{e0}
  \StateVar[E|1]{(2.25,0)}{e1}
  \StateVar[E|2]{(4.5,0)}{e2}
}

\VCPut{(5,-4)} {
  \StateVar[F|0]{(0,0)}{f0}
  \StateVar[F|1]{(2.25,0)}{f1}
  \StateVar[F|2]{(4.5,0)}{f2}
}

\VCPut{(12.4,-4)} {
  \StateVar[G|0]{(0,0)}{g0}
  \StateVar[G|1]{(2.25,0)}{g1}
  \StateVar[G|2]{(4.5,0)}{g2}
}

% initial--final
\Initial[n]{a}
\Final[e]{f2}



% transitions
\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3}
\ChgEdgeArrowWidth{7pt}
\EdgeR{ae}{cw}{}
\VCurveR{angleA=0,angleB=90,ncurv=0.9}{b}{e2}{}
\EdgeR{cw}{g0}{}
%\VCurveR{angleA=0,angleB=0,ncurv=1}{e0}{g20}{}
\DimEdge
\EdgeR{aw}{be}{}
\VCurveR{angleA=180,angleB=90,ncurv=0.9}{b}{d0}{}
\VCurveR{angleA=180,angleB=90,ncurv=1.2}{c}{f1}{}
%\VCurveR{angleA=0,angleB=-90,ncurv=0.6}{e1}{d10}{}
%\VCurveR{angleA=180,angleB=-90,ncurv=0.6}{e0}{f00}{}



\RstEdge
\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3}
\ChgEdgeArrowWidth{7pt}


\VCurveL{angleA=-45,angleB=-145,ncurv=1}{d1e}{d2w}{} 
\VCurveL{angleB=35,angleA=135,ncurv=1}{d2w}{d1e}{}
\CLoopS{d0}{}
\VCurveL{angleA=-45,angleB=-145,ncurv=1}{e1e}{e2w}{} 
\VCurveL{angleB=35,angleA=135,ncurv=1}{e2w}{e1e}{}
\CLoopS{e0}{}
\VCurveL{angleA=-45,angleB=-145,ncurv=1}{f1e}{f2w}{} 
\VCurveL{angleB=35,angleA=135,ncurv=1}{f2w}{f1e}{}
\CLoopS{f0}{}
\VCurveL{angleA=-45,angleB=-145,ncurv=1}{g1e}{g2w}{} 
\VCurveL{angleB=35,angleA=135,ncurv=1}{g2w}{g1e}{}
\CLoopS{g0}{}
\DimEdge
\VCurveL{angleA=-45,angleB=-145,ncurv=1}{d0e}{d1w}{} 
\VCurveL{angleB=35,angleA=135,ncurv=1}{d1w}{d0e}{}
\CLoopS{d2}{}
\VCurveL{angleA=-45,angleB=-145,ncurv=1}{e0e}{e1w}{} 
\VCurveL{angleB=35,angleA=135,ncurv=1}{e1w}{e0e}{}
\CLoopS{e2}{}
\VCurveL{angleA=-45,angleB=-145,ncurv=1}{f0e}{f1w}{} 
\VCurveL{angleB=35,angleA=135,ncurv=1}{f1w}{f0e}{}
\CLoopS{f2}{}
\VCurveL{angleA=-45,angleB=-145,ncurv=1}{g0e}{g1w}{} 
\VCurveL{angleB=35,angleA=135,ncurv=1}{g1w}{g0e}{}
\CLoopS{g2}{}
%\VArcR[.5]{arcangle=40,ncurv=1.0}{g20}{g01}{}
%\VArcR[.5]{arcangle=40,ncurv=1.0}{g01}{g20}{}
%\EdgeBorder
%\ArcR{g00}{g11}{} \ArcR{g11}{g00}{}
%\ArcR{g10}{g21}{} \ArcR{g21}{g10}{}
%\EdgeBorderOff
%\DimEdge
%\ArcR{g00}{g01}{} \ArcR{g01}{g00}{}
%\ArcR{g10}{g11}{} \ArcR{g11}{g10}{}
%\ArcR{g20}{g21}{} \ArcR{g21}{g20}{}

\end{VCPicture}
% }
% \renewcommand{\frcurrentcaption}{Automate reconnaissant les entiers congrus à 5 modulo 12 en base 2}
% \renewcommand{\encurrentcaption}{Automate accepting integers congruent to 5 modulo 12 in base 2}


==> aut_sup5_2.tex <==

% \SmallPicture\VCDraw{
\begin{VCPicture}{(-2,-12)(16,2)}

% states
  \State[0]{(0,0)}{e}

  \State[0]{(0,-2)}{e0}
  \State[1]{(2,-2)}{e1}

  \State[0]{(0,-4)}{e00}
  \State[1]{(2,-4)}{e10}
  \State[2]{(4,-4)}{e01}
  \State[3]{(6,-4)}{e11}

  \State[0]{(0,-8)}{e000}
  \State[1]{(2,-8)}{e100}
  \State[2]{(4,-8)}{e010}
  \State[3]{(6,-8)}{e110}
  \State[4]{(8,-8)}{e001}
  \State[5]{(10,-8)}{e101}
  \State[6]{(12,-8)}{e011}
  \State[7]{(14,-8)}{e111}

  \StateVar[\geq 5]{(10,-10)}{top}
\Initial[nw]{e}
\Final[s]{top}
\Final[se]{e101}
\Final[se]{e011}
\Final[se]{e111}
\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3}
\ChgEdgeArrowWidth{7pt}

\EdgeR{e}{e1}{}
\EdgeR{e0}{e01}{}
\EdgeR{e1}{e11}{}
\EdgeR{e00}{e001}{}
\EdgeR{e01}{e011}{}
\EdgeR{e10}{e101}{}
\EdgeR{e11}{e111}{}
\VCurveR{angleA=-90,angleB=180,ncurv=0.4}{e000}{top}{}
\VCurveR{angleA=-90,angleB=180,ncurv=0.5}{e100}{top}{}
\VCurveR{angleA=-90,angleB=180,ncurv=0.7}{e010}{top}{}
\VCurveR{angleA=-90,angleB=180}{e110}{top}{}
\VCurveR{angleA=-90,angleB=180}{e001}{top}{}
\EdgeR{e101}{top}{}
\VCurveR{angleA=-90,angleB=0}{e111}{top}{}
\VCurveR{angleA=-90,angleB=0}{e011}{top}{}
\CLoopSE{top}{}

\DimEdge
\CLoopSW{top}{}
\EdgeR{e}{e0}{}\EdgeR{e0}{e00}{}\EdgeR{e00}{e000}{}\CLoopSW{e000}{}
               \EdgeR{e1}{e10}{}\EdgeR{e10}{e100}{}\CLoopSW{e100}{}
                                \EdgeR{e01}{e010}{}\CLoopSW{e010}{}
                                \EdgeR{e11}{e110}{}\CLoopSW{e110}{}
                                                   \CLoopSW{e111}{}
                                                   \CLoopSW{e001}{}
                                                   \CLoopSW{e011}{}
                                                   \CLoopSW{e101}{}
\pcline[linestyle=dashed]{-}(8.6,0.5)(8.6,-11.5)
%\LoopN{A}{a} \LoopS{C}{d}
%
\end{VCPicture}
% }
% 
% \renewcommand\frcurrentcaption{$n\geq5$}
% \renewcommand\encurrentcaption{$n\geq5$}

==> general_case_after_product.tex <==

% \SmallPicture\VCDraw{
\begin{VCPicture}{(-2,-14)(18,1)}
\newgray{ginw}{0.95}
\psdots[dotsize=1pt,linecolor=ginw](-2,-13)
\psdots[dotsize=1pt,linecolor=ginw](18,1)
\StateVar[A|\epsilon]{(0,0)}{e}
\StateVar[B|0]{(2,-4)}{e0}
\StateVar[B|00]{(4,-4)}{e00}
\StateVar[B|0,1]{(8,-4)}{e000}
\StateVar[B|0,0]{(8,-6)}{e0000}

\VCPut{(8,-12)}{ %end
  \StateVar[D|0,0]{(0,0)}{s00}
  \StateVar[D|0,1]{(0,2)}{s01}
  \StateVar[D|1,0]{(3,0)}{s10}
  \StateVar[D|1,1]{(3,2)}{s11}
  \StateVar[D|2,0]{(6,0)}{s20}
  \StateVar[D|2,1]{(6,2)}{s21}
}

\Initial[nw]{ew}
\Final[s]{s00}\Final[n]{s01}

\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3}
\ChgEdgeArrowWidth{7pt}

\VArcR[.5]{arcangle=32,ncurv=1.4}{s20}{s01}{}
\VArcR[.5]{arcangle=32,ncurv=1.4}{s01}{s20}{}
%\ArcR{20}{01}{} \ArcR{01}{20}{}

\ArcR{s00}{s11}{} \ArcR{s11}{s00}{}
\ArcR{s10}{s21}{} \ArcR{s21}{s10}{}
\VCurveR{angleA=0,angleB=90}{e0000}{s11}{}
\VCurveR{angleA=0,angleB=0}{e000}{s20}{}

\DimEdge
\EdgeR{e}{e0}{}
\EdgeR{e0}{e00}{}
\EdgeR{e00}{e000}{}
\ArcR{e000}{e0000}{}
\ArcR{e0000}{e000}{}
\ArcR{s00}{s01}{} \ArcR{s01}{s00}{}
\ArcR{s10}{s11}{} \ArcR{s11}{s10}{}
\ArcR{s20}{s21}{} \ArcR{s21}{s20}{}

\end{VCPicture}
% }


==> general_case_before_product1.tex <==

% \SmallPicture\VCDraw{
\begin{VCPicture}{(-3,-14)(3,1)}

% states
  \State[A]{(0,0)}{e}

  \State[B]{(-2,-5)}{e0}
  \State[C]{(2,-5)}{e1}

  \StateVar[D]{(0,-12)}{top}
\Initial[n]{e}
\Final[s]{top}
\Final[s]{e1}
\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3}
\ChgEdgeArrowWidth{7pt}

\EdgeR{e}{e1}{}
\EdgeR{e1}{top}{}
\EdgeR{e0}{top}{}
\CLoopSE{top}{}
\DimEdge
\CLoopSW{top}{}
\EdgeR{e}{e0}{}
\CLoopW{e0}{}
\CLoopW{e1}{}
%\pcline[linestyle=dashed]{-}(8.6,0.5)(8.6,-11.5)
%\LoopN{A}{a} \LoopS{C}{d}
%
\end{VCPicture}
% }


==> general_case_before_product2.tex <==

% \SmallPicture\VCDraw{
\begin{VCPicture}{(-2,-4)(18,1)}
\newgray{ginw}{0.95}
\psdots[dotsize=1pt,linecolor=ginw](-2,-3)
\psdots[dotsize=1pt,linecolor=ginw](18,1)
\StateVar[\epsilon]{(0,0)}{e}
\StateVar[0]{(2,0)}{e0}
\StateVar[00]{(4,0)}{e00}

\VCPut{(8,-2)}{ %end
  \StateVar[0,0]{(0,0)}{s00}
  \StateVar[0,1]{(0,2)}{s01}
  \StateVar[1,0]{(3,0)}{s10}
  \StateVar[1,1]{(3,2)}{s11}
  \StateVar[2,0]{(6,0)}{s20}
  \StateVar[2,1]{(6,2)}{s21}
}
% initial--final
\Initial[w]{e}
\Final[s]{s00}\Final[n]{s01}
\Final[s]{e}\Final[s]{e0}\Final[s]{e00}
% transitions
\FixDimEdge{solid}{1}{black}{black}
\ChgEdgeLineWidth{3}
\ChgEdgeArrowWidth{7pt}

\VArcR[.5]{arcangle=32,ncurv=1.4}{s20}{s01}{}
\VArcR[.5]{arcangle=32,ncurv=1.4}{s01}{s20}{}
%\ArcR{20}{01}{} \ArcR{01}{20}{}

\ArcR{s00}{s11}{} \ArcR{s11}{s00}{}
\ArcR{s10}{s21}{} \ArcR{s21}{s10}{}

\DimEdge
\EdgeR{e}{e0}{}
\EdgeR{e0}{e00}{}
\EdgeR{e00}{s01}{}
\ArcR{s00}{s01}{} \ArcR{s01}{s00}{}
\ArcR{s10}{s11}{} \ArcR{s11}{s10}{}
\ArcR{s20}{s21}{} \ArcR{s21}{s20}{}

\end{VCPicture}
% }


==> up_criterion.vcsg.tex <==
\begin{VCPicture}{(14,-9)(19,11)}

\pspolygon[linecolor=black,linewidth=1pt,linestyle=solid](3,0)(15.5,-5.5)(15.5,5.5)
\rput[c]{0}(9,10){\scalebox{2}{D.A.G.}}
\VCPut{(15,-5.25)}{
  \HideState
  \State{(0.5,0)}{T1}
  \State{(0,1.5)}{T2}
  \State{(0,3)}{T3}
  \State{(0,4.5)}{T4}
  \State{(0,6)}{T5}
  \State{(0,7.5)}{T6}
  \State{(0,9)}{T7}
  \State{(0,10.5)}{T8}
}

\VCPut{(29,-6)}{

%   \LargeState
  \rput[c]{0}(0,16){\scalebox{2}{Type 1 SCC's}}
  \rput[c]{0}(0,15.25){\scalebox{2}{(Pascal)}}
  \State[\bot]{(0,-1)}{P1}
  \pnode(-6,-2){P1b}
  \pnode(-0.5,-1.5){P1c}
  
  \FixStateDiameter{2.5cm}
  \SquareStates
  \State{(0,3)}{P2}
  \State{(0,8)}{P3}  
  
  \HideState
  \State{(0,7)}{P3b}
  \ShowState
  \State{(0,13)}{P4}  
  
  \FixStateDiameter{0.8cm}
  \OvalStates
  
  \ChgOvalStateRatio{0.2}
  \State{(-0.7,2.5)}{Q2}      
  
  \ChgOvalStateRatio{1.5}
  \State{(0.25,3.5)}{Q2b}
  
  \ChgOvalStateRatio{2}
  \State{(0,8.5)}{Q3}
  
  \ChgOvalStateRatio{2.5}
  \State{(0,12.5)}{Q4}
}



\VCPut{(22,-6)}{ 
  \rput[c]{0}(0,16){\scalebox{2}{Type 2 SCC's}} 
  \rput[c]{0}(0,15.25){\scalebox{2}{(0-circuits)}}
  \State{(0,1)}{O1}
  
  \FixStateDiameter{0.8cm}
  \OvalStates
  \ChgOvalStateRatio{0.2}
  \State{(0,3)}{O2}      
  
  \ChgOvalStateRatio{1.5}
  \State{(0,5.25)}{O2b}
  
  \ChgOvalStateRatio{2}
  \State{(0,9)}{O3}
  
  \ChgOvalStateRatio{2.5}
  \State{(0,13)}{O4}
}

\SetEdgeArrowWidthCoef{6}
\NodeSeparationOn
\ChgNodeSep{4}

% \ncline{T1}(28,-8)
\EdgeR{T2}{O1}{}
% \VCurveR{angleA=-20,angleB=225,ncurv=1}{P1b}{P1}{}
\EdgeR{T3}{O2}{}
\EdgeR{T4}{O2b}{}
\EdgeR{T5}{P3b}{}
\EdgeR{T6}{O3}{}
\EdgeR{T7}{O3}{}
\EdgeR{T8}{O4}{}
% \EdgeR{



\newcommand{\isomorphicStates}[2]{
  \VCurveR{angleA=90,angleB=90,ncurv=0}{#1}{#2}{}
  \VCurveR{angleA=270,angleB=270,ncurv=0}{#1}{#2}{}
}


\NodeSeparationOff
\VCurveR{angleA=-18,angleB=225,ncurv=1}{P1b}{P1c}{}
\PlainEdge
\EdgeR{T1}{P1b}{}
\ChgEdgeLineStyle{dashed}




\isomorphicStates{O1}{P1}
\isomorphicStates{O2}{Q2}
\isomorphicStates{O2b}{Q2b}
\isomorphicStates{O3}{Q3}
\isomorphicStates{O4}{Q4}




\end{VCPicture}

==> up_example.tex <==
%\centering
% \SmallPicture\VCDraw{
\begin{VCPicture}{(-4,-8)(20,3)}



\State[\epsilon]{(-2,0)}{dage}
\State[0]{(0,2)}{dag0}
\State[1]{(0,-2)}{dag1}
\StateVar[11]{(2,-4)}{dag11}
\StateVar[B_2]{(8,0.5)}{cb2}
\StateVar[C_2]{(8,-1.5)}{cc2}
\StateVar[D_2]{(8,-6)}{cd2}
\StateVar[A]{(16,2.5)}{pa}
\StateVar[B]{(16,0.5)}{pb}
\StateVar[C]{(16,-1.5)}{pc}


\Initial{dage}

\VCPut{(14,-5.5)}{
\pspolygon[linearc=0](4.7,-2.1)(-1.7,-2.1)(-1.7,2.1)(4.7,2.1)
\StateVar[D]{(-1,-1)}{pd}
\StateVar[E]{(1,0)}{pe}
\StateVar[F]{(2.5,-1.5)}{pf}
\StateVar[G]{(2.5,1.5)}{pg}
\StateVar[H]{(4,0)}{ph}
}
\Initial{dage}
\Final{pb}
\Final{pc}
\Final[e]{cd2}
\Final{dag11}
\Final[ne]{pge}
\Final[e]{ph}
% \Final[se]{pf}
\Final[nw]{pew}


\pspolygon[linearc=0](16.6,4.1)(15.4,4.1)(15.4,-3.1)(16.6,-3.1)

\ChgEdgeLineWidth{3}
\ChgEdgeArrowWidth{7pt}
\FixDimEdge{solid}{1}{black}{black}



% \pcline[linewidth=2pt,linestyle=dotted]{-}(8,1.43)(16,1.43)
% \pcline[linewidth=2pt,linestyle=dotted]{-}(8,-1.43)(16,-1.43)
% \pcline[linewidth=2pt,linestyle=dotted]{-}(8,-6.43)(13,-7.45)
% \pcline[linewidth=2pt,linestyle=dotted]{-}(8,-5.57)(13,-6.55)

\EdgeR{dag0}{pa}{}
\EdgeR{dage}{dag1}{}
\CLoopS{phw}{}
\EdgeR{cb2e}{pa}{}
\VCurveL{angleA=-30,angleB=210,ncurv=0.65}{cc2e}{pc}{}
\ArcR{pa}{pb}{}
\ArcR{pb}{pa}{}
\CLoopS{pc}{}
\EdgeR{dag1}{dag11w}{}
\ArcR{pee}{pde}{}\ArcR{pgw}{pee}{}
\VCurveL{angleA=-45,angleB=-160,ncurv=0.65}{pde}{pfw}{}\EdgeR{pfw}{pg}{}
\VCurveL{angleA=-45,angleB=-160,ncurv=0.65}{cd2e}{pfw}{}
\DimEdge
\EdgeR{dag11e}{cd2w}{}
\CLoopN{cd2}{}
\CLoopN{pde}{}
\ArcR{pb}{pc}{}
\ArcR{pc}{pb}{}
\CLoopN{pa}{}
\EdgeR{dage}{dag0}{}
\ArcR{cb2}{cc2}{}
\ArcR{cc2}{cb2}{}
\EdgeR{dag1}{cc2w}{}
\EdgeR{pge}{phw}{}\ArcR{pee}{pgw}{}\EdgeR{pfw}{pee}{}\EdgeR{phw}{pfe}{}



%%%%%%%%%%%%%%%%%%%%%%%% Dotted lines
\NodeSeparationOff
\VCurveR{angleA=-18,angleB=225,ncurv=1}{P1b}{P1c}{}
\PlainEdge
\EdgeR{T1}{P1b}{}
\ChgEdgeLineStyle{dotted}
\VCurveR{angleA=90,angleB=90,ncurv=0,linewidth=2.5pt}{cd2e}{pd}{}
\VCurveR{angleA=270,angleB=270,ncurv=0,linewidth=2.5pt}{cd2w}{pd}{}
\VCurveR{angleA=90,angleB=90,ncurv=0,linewidth=2.5pt}{cb2e}{pb}{}
\VCurveR{angleA=270,angleB=270,ncurv=0,linewidth=2.5pt}{cc2e}{pc}{}
\end{VCPicture}
% }
% \renewcommand\frcurrentcaption{Un exemple complet du critère UP}
% \renewcommand\encurrentcaption{A complete example of the UP criterion}


